Search for the doubly charmed baryon $\it{\Omega}_{cc}^{+}$

A search for the doubly charmed baryon $\it{\Omega}_{cc}^{+}$ with the decay mode $\it{\Omega}_{cc}^{+}\to\it{\Xi}_c^{+}K^{-}\pi^{+}$ is performed using proton-proton collision data at a centre-of-mass energy of 13$\mathrm{\,Te\kern -0.1em V}$ collected by the LHCb experiment from 2016 to 2018, corresponding to an integrated luminosity of $5.4\,\mathrm{fb}^{-1}$. No significant signal is observed within the invariant mass range of 3.6 to 4.0$\mathrm{\,Ge\kern -0.1em V}/c^2$. Upper limits are set on the ratio $R$ of the production cross-section times the total branching fraction of the $\it{\Omega}_{cc}^{+}\to\it{\Xi}_c^{+}K^{-}\pi^{+}$ decay with respect to the $\it{\Xi}_{cc}^{++}\to\it{\Lambda}_c^{+}K^{-}\pi^{+}\pi^{+}$ decay. Upper limits at 95% credibility level for $R$ in the range $0.005$ to $0.11$ are obtained for different hypotheses on the $\it{\Omega}_{cc}^{+}$ mass and lifetime in the rapidity range from 2.0 to 4.5 and transverse momentum range from 4 to 15$\mathrm{\,Ge\kern -0.1em V}/c$.

==> Authorship_LHCb-PAPER-2021-011-arXiv.tex <==
LHCb collaboration:
R. Aaij,
C. Abell{\'a}n Beteta,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista Leite,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
S. Bifani,
P. Billoir,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
L. Calero Diaz,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
K. Carvalho Akiba,
A. Casais Vidal,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
J. Cerasoli,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
J.A. de Vries,
C.T. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Cicco,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
H. Dijkstra,
V. Dobishuk,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
K. Dreimanis,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
A. Falabella,
J. Fan,
Y. Fan,
B. Fang,
S. Farry,
D. Fazzini,
M. F{\'e}o,
A. Fernandez Prieto,
J.M. Fernandez-tenllado Arribas,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
A. Fkiaras,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
W. Funk,
E. Gabriel,
T. Gaintseva,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
H.K. Giemza,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
L. Giubega,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
P. Griffith,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
T. Halewood-leagas,
P.M. Hamilton,
J.P. Hammerich,
Q. Han,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
M. Jezabek,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
M. Karpov,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
L. Li,
P. Li,
S. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
S. Liu,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
G.H. Lovell,
Y. Lu,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Madejczyk,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
G. Meier,
N. Meinert,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
I. Neri,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
D.P. O'Hanlon,
R. Oldeman,
M.E. Olivares,
C.J.G. Onderwater,
R.H. O'neil,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
C.J. Parkinson,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
M. Petric,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
T.T.H. Pham,
A. Philippov,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
Resmi  P.K,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
H. Pullen,
G. Punzi,
H. Qi,
W. Qian,
J. Qin,
N. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
S. Ricciardi,
K. Rinnert,
P. Robbe,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
D. Sanchez Gonzalo,
C. Sanchez Gras,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
P. Seyfert,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
V. Shevchenko,
E.B. Shields,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
I. Slazyk,
J.C. Smallwood,
J.G. Smeaton,
A. Smetkina,
E. Smith,
M. Smith,
A. Snoch,
M. Soares,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
S. Stone,
M.E. Stramaglia,
M. Straticiuc,
D. Strekalina,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
A.R. Tanner,
A. Terentev,
F. Teubert,
E. Thomas,
K.A. Thomson,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
D. Torres Machado,
D.Y. Tou,
M.T. Tran,
E. Trifonova,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
M. Van Dijk,
E. van Herwijnen,
C.B. Van Hulse,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
K. Vos,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
H.M. Wark,
N.K. Watson,
S.G. Weber,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
D. Wiedner,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
X. Zhou,
Y. Zhou,
X. Zhu,
Z. Zhu,
V. Zhukov,
J.B. Zonneveld,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica


==> Authorship_LHCb-PAPER-2021-011.tex <==
% LHCb collaboration author list
% Data extracted on May 12th, 2021 at 3:40pm for paper reference LHCb-PAPER-2021-011
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{32}$,
C.~Abell{\'a}n~Beteta$^{50}$,
T.~Ackernley$^{60}$,
B.~Adeva$^{46}$,
M.~Adinolfi$^{54}$,
H.~Afsharnia$^{9}$,
C.A.~Aidala$^{86}$,
S.~Aiola$^{25}$,
Z.~Ajaltouni$^{9}$,
S.~Akar$^{65}$,
J.~Albrecht$^{15}$,
F.~Alessio$^{48}$,
M.~Alexander$^{59}$,
A.~Alfonso~Albero$^{45}$,
Z.~Aliouche$^{62}$,
G.~Alkhazov$^{38}$,
P.~Alvarez~Cartelle$^{55}$,
S.~Amato$^{2}$,
Y.~Amhis$^{11}$,
L.~An$^{48}$,
L.~Anderlini$^{22}$,
A.~Andreianov$^{38}$,
M.~Andreotti$^{21}$,
F.~Archilli$^{17}$,
A.~Artamonov$^{44}$,
M.~Artuso$^{68}$,
K.~Arzymatov$^{42}$,
E.~Aslanides$^{10}$,
M.~Atzeni$^{50}$,
B.~Audurier$^{12}$,
S.~Bachmann$^{17}$,
M.~Bachmayer$^{49}$,
J.J.~Back$^{56}$,
P.~Baladron~Rodriguez$^{46}$,
V.~Balagura$^{12}$,
W.~Baldini$^{21}$,
J.~Baptista~Leite$^{1}$,
R.J.~Barlow$^{62}$,
S.~Barsuk$^{11}$,
W.~Barter$^{61}$,
M.~Bartolini$^{24}$,
F.~Baryshnikov$^{83}$,
J.M.~Basels$^{14}$,
G.~Bassi$^{29}$,
B.~Batsukh$^{68}$,
A.~Battig$^{15}$,
A.~Bay$^{49}$,
M.~Becker$^{15}$,
F.~Bedeschi$^{29}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{68}$,
V.~Belavin$^{42}$,
S.~Belin$^{27}$,
V.~Bellee$^{49}$,
K.~Belous$^{44}$,
I.~Belov$^{40}$,
I.~Belyaev$^{41}$,
G.~Bencivenni$^{23}$,
E.~Ben-Haim$^{13}$,
A.~Berezhnoy$^{40}$,
R.~Bernet$^{50}$,
D.~Berninghoff$^{17}$,
H.C.~Bernstein$^{68}$,
C.~Bertella$^{48}$,
A.~Bertolin$^{28}$,
C.~Betancourt$^{50}$,
F.~Betti$^{48}$,
Ia.~Bezshyiko$^{50}$,
S.~Bhasin$^{54}$,
J.~Bhom$^{35}$,
L.~Bian$^{73}$,
M.S.~Bieker$^{15}$,
S.~Bifani$^{53}$,
P.~Billoir$^{13}$,
M.~Birch$^{61}$,
F.C.R.~Bishop$^{55}$,
A.~Bitadze$^{62}$,
A.~Bizzeti$^{22,k}$,
M.~Bj{\o}rn$^{63}$,
M.P.~Blago$^{48}$,
T.~Blake$^{56}$,
F.~Blanc$^{49}$,
S.~Blusk$^{68}$,
D.~Bobulska$^{59}$,
J.A.~Boelhauve$^{15}$,
O.~Boente~Garcia$^{46}$,
T.~Boettcher$^{65}$,
A.~Boldyrev$^{82}$,
A.~Bondar$^{43}$,
N.~Bondar$^{38,48}$,
S.~Borghi$^{62}$,
M.~Borisyak$^{42}$,
M.~Borsato$^{17}$,
J.T.~Borsuk$^{35}$,
S.A.~Bouchiba$^{49}$,
T.J.V.~Bowcock$^{60}$,
A.~Boyer$^{48}$,
C.~Bozzi$^{21}$,
M.J.~Bradley$^{61}$,
S.~Braun$^{66}$,
A.~Brea~Rodriguez$^{46}$,
M.~Brodski$^{48}$,
J.~Brodzicka$^{35}$,
A.~Brossa~Gonzalo$^{56}$,
D.~Brundu$^{27}$,
A.~Buonaura$^{50}$,
C.~Burr$^{48}$,
A.~Bursche$^{72}$,
A.~Butkevich$^{39}$,
J.S.~Butter$^{32}$,
J.~Buytaert$^{48}$,
W.~Byczynski$^{48}$,
S.~Cadeddu$^{27}$,
H.~Cai$^{73}$,
R.~Calabrese$^{21,f}$,
L.~Calefice$^{15,13}$,
L.~Calero~Diaz$^{23}$,
S.~Cali$^{23}$,
R.~Calladine$^{53}$,
M.~Calvi$^{26,j}$,
M.~Calvo~Gomez$^{85}$,
P.~Camargo~Magalhaes$^{54}$,
P.~Campana$^{23}$,
A.F.~Campoverde~Quezada$^{6}$,
S.~Capelli$^{26,j}$,
L.~Capriotti$^{20,d}$,
A.~Carbone$^{20,d}$,
G.~Carboni$^{31}$,
R.~Cardinale$^{24}$,
A.~Cardini$^{27}$,
I.~Carli$^{4}$,
P.~Carniti$^{26,j}$,
L.~Carus$^{14}$,
K.~Carvalho~Akiba$^{32}$,
A.~Casais~Vidal$^{46}$,
G.~Casse$^{60}$,
M.~Cattaneo$^{48}$,
G.~Cavallero$^{48}$,
S.~Celani$^{49}$,
J.~Cerasoli$^{10}$,
A.J.~Chadwick$^{60}$,
M.G.~Chapman$^{54}$,
M.~Charles$^{13}$,
Ph.~Charpentier$^{48}$,
G.~Chatzikonstantinidis$^{53}$,
C.A.~Chavez~Barajas$^{60}$,
M.~Chefdeville$^{8}$,
C.~Chen$^{3}$,
S.~Chen$^{4}$,
A.~Chernov$^{35}$,
V.~Chobanova$^{46}$,
S.~Cholak$^{49}$,
M.~Chrzaszcz$^{35}$,
A.~Chubykin$^{38}$,
V.~Chulikov$^{38}$,
P.~Ciambrone$^{23}$,
M.F.~Cicala$^{56}$,
X.~Cid~Vidal$^{46}$,
G.~Ciezarek$^{48}$,
P.E.L.~Clarke$^{58}$,
M.~Clemencic$^{48}$,
H.V.~Cliff$^{55}$,
J.~Closier$^{48}$,
J.L.~Cobbledick$^{62}$,
V.~Coco$^{48}$,
J.A.B.~Coelho$^{11}$,
J.~Cogan$^{10}$,
E.~Cogneras$^{9}$,
L.~Cojocariu$^{37}$,
P.~Collins$^{48}$,
T.~Colombo$^{48}$,
L.~Congedo$^{19,c}$,
A.~Contu$^{27}$,
N.~Cooke$^{53}$,
G.~Coombs$^{59}$,
G.~Corti$^{48}$,
C.M.~Costa~Sobral$^{56}$,
B.~Couturier$^{48}$,
D.C.~Craik$^{64}$,
J.~Crkovsk\'{a}$^{67}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{58}$,
C.L.~Da~Silva$^{67}$,
S.~Dadabaev$^{83}$,
E.~Dall'Occo$^{15}$,
J.~Dalseno$^{46}$,
C.~D'Ambrosio$^{48}$,
A.~Danilina$^{41}$,
P.~d'Argent$^{48}$,
A.~Davis$^{62}$,
O.~De~Aguiar~Francisco$^{62}$,
K.~De~Bruyn$^{79}$,
S.~De~Capua$^{62}$,
M.~De~Cian$^{49}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{19,c}$,
D.~De~Simone$^{50}$,
P.~De~Simone$^{23}$,
J.A.~de~Vries$^{80}$,
C.T.~Dean$^{67}$,
D.~Decamp$^{8}$,
L.~Del~Buono$^{13}$,
B.~Delaney$^{55}$,
H.-P.~Dembinski$^{15}$,
A.~Dendek$^{34}$,
V.~Denysenko$^{50}$,
D.~Derkach$^{82}$,
O.~Deschamps$^{9}$,
F.~Desse$^{11}$,
F.~Dettori$^{27,e}$,
B.~Dey$^{77}$,
A.~Di~Cicco$^{23}$,
P.~Di~Nezza$^{23}$,
S.~Didenko$^{83}$,
L.~Dieste~Maronas$^{46}$,
H.~Dijkstra$^{48}$,
V.~Dobishuk$^{52}$,
A.M.~Donohoe$^{18}$,
F.~Dordei$^{27}$,
A.C.~dos~Reis$^{1}$,
L.~Douglas$^{59}$,
A.~Dovbnya$^{51}$,
A.G.~Downes$^{8}$,
K.~Dreimanis$^{60}$,
M.W.~Dudek$^{35}$,
L.~Dufour$^{48}$,
V.~Duk$^{78}$,
P.~Durante$^{48}$,
J.M.~Durham$^{67}$,
D.~Dutta$^{62}$,
A.~Dziurda$^{35}$,
A.~Dzyuba$^{38}$,
S.~Easo$^{57}$,
U.~Egede$^{69}$,
V.~Egorychev$^{41}$,
S.~Eidelman$^{43,v}$,
S.~Eisenhardt$^{58}$,
S.~Ek-In$^{49}$,
L.~Eklund$^{59,w}$,
S.~Ely$^{68}$,
A.~Ene$^{37}$,
E.~Epple$^{67}$,
S.~Escher$^{14}$,
J.~Eschle$^{50}$,
S.~Esen$^{13}$,
T.~Evans$^{48}$,
A.~Falabella$^{20}$,
J.~Fan$^{3}$,
Y.~Fan$^{6}$,
B.~Fang$^{73}$,
S.~Farry$^{60}$,
D.~Fazzini$^{26,j}$,
M.~F{\'e}o$^{48}$,
A.~Fernandez~Prieto$^{46}$,
J.M.~Fernandez-tenllado~Arribas$^{45}$,
A.D.~Fernez$^{66}$,
F.~Ferrari$^{20,d}$,
L.~Ferreira~Lopes$^{49}$,
F.~Ferreira~Rodrigues$^{2}$,
S.~Ferreres~Sole$^{32}$,
M.~Ferrillo$^{50}$,
M.~Ferro-Luzzi$^{48}$,
S.~Filippov$^{39}$,
R.A.~Fini$^{19}$,
M.~Fiorini$^{21,f}$,
M.~Firlej$^{34}$,
K.M.~Fischer$^{63}$,
D.S.~Fitzgerald$^{86}$,
C.~Fitzpatrick$^{62}$,
T.~Fiutowski$^{34}$,
A.~Fkiaras$^{48}$,
F.~Fleuret$^{12}$,
M.~Fontana$^{13}$,
F.~Fontanelli$^{24,h}$,
R.~Forty$^{48}$,
V.~Franco~Lima$^{60}$,
M.~Franco~Sevilla$^{66}$,
M.~Frank$^{48}$,
E.~Franzoso$^{21}$,
G.~Frau$^{17}$,
C.~Frei$^{48}$,
D.A.~Friday$^{59}$,
J.~Fu$^{25}$,
Q.~Fuehring$^{15}$,
W.~Funk$^{48}$,
E.~Gabriel$^{32}$,
T.~Gaintseva$^{42}$,
A.~Gallas~Torreira$^{46}$,
D.~Galli$^{20,d}$,
S.~Gambetta$^{58,48}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{25}$,
Y.~Gao$^{5}$,
M.~Garau$^{27}$,
L.M.~Garcia~Martin$^{56}$,
P.~Garcia~Moreno$^{45}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{26,j}$,
B.~Garcia~Plana$^{46}$,
F.A.~Garcia~Rosales$^{12}$,
L.~Garrido$^{45}$,
C.~Gaspar$^{48}$,
R.E.~Geertsema$^{32}$,
D.~Gerick$^{17}$,
L.L.~Gerken$^{15}$,
E.~Gersabeck$^{62}$,
M.~Gersabeck$^{62}$,
T.~Gershon$^{56}$,
D.~Gerstel$^{10}$,
Ph.~Ghez$^{8}$,
V.~Gibson$^{55}$,
H.K.~Giemza$^{36}$,
M.~Giovannetti$^{23,p}$,
A.~Giovent{\`u}$^{46}$,
P.~Gironella~Gironell$^{45}$,
L.~Giubega$^{37}$,
C.~Giugliano$^{21,f,48}$,
K.~Gizdov$^{58}$,
E.L.~Gkougkousis$^{48}$,
V.V.~Gligorov$^{13}$,
C.~G{\"o}bel$^{70}$,
E.~Golobardes$^{85}$,
D.~Golubkov$^{41}$,
A.~Golutvin$^{61,83}$,
A.~Gomes$^{1,a}$,
S.~Gomez~Fernandez$^{45}$,
F.~Goncalves~Abrantes$^{63}$,
M.~Goncerz$^{35}$,
G.~Gong$^{3}$,
P.~Gorbounov$^{41}$,
I.V.~Gorelov$^{40}$,
C.~Gotti$^{26}$,
E.~Govorkova$^{48}$,
J.P.~Grabowski$^{17}$,
T.~Grammatico$^{13}$,
L.A.~Granado~Cardoso$^{48}$,
E.~Graug{\'e}s$^{45}$,
E.~Graverini$^{49}$,
G.~Graziani$^{22}$,
A.~Grecu$^{37}$,
L.M.~Greeven$^{32}$,
P.~Griffith$^{21,f}$,
L.~Grillo$^{62}$,
S.~Gromov$^{83}$,
B.R.~Gruberg~Cazon$^{63}$,
C.~Gu$^{3}$,
M.~Guarise$^{21}$,
P. A.~G{\"u}nther$^{17}$,
E.~Gushchin$^{39}$,
A.~Guth$^{14}$,
Y.~Guz$^{44}$,
T.~Gys$^{48}$,
T.~Hadavizadeh$^{69}$,
G.~Haefeli$^{49}$,
C.~Haen$^{48}$,
J.~Haimberger$^{48}$,
T.~Halewood-leagas$^{60}$,
P.M.~Hamilton$^{66}$,
J.P.~Hammerich$^{60}$,
Q.~Han$^{7}$,
X.~Han$^{17}$,
T.H.~Hancock$^{63}$,
S.~Hansmann-Menzemer$^{17}$,
N.~Harnew$^{63}$,
T.~Harrison$^{60}$,
C.~Hasse$^{48}$,
M.~Hatch$^{48}$,
J.~He$^{6,b}$,
M.~Hecker$^{61}$,
K.~Heijhoff$^{32}$,
K.~Heinicke$^{15}$,
A.M.~Hennequin$^{48}$,
K.~Hennessy$^{60}$,
L.~Henry$^{48}$,
J.~Heuel$^{14}$,
A.~Hicheur$^{2}$,
D.~Hill$^{49}$,
M.~Hilton$^{62}$,
S.E.~Hollitt$^{15}$,
J.~Hu$^{17}$,
J.~Hu$^{72}$,
W.~Hu$^{7}$,
X.~Hu$^{3}$,
W.~Huang$^{6}$,
X.~Huang$^{73}$,
W.~Hulsbergen$^{32}$,
R.J.~Hunter$^{56}$,
M.~Hushchyn$^{82}$,
D.~Hutchcroft$^{60}$,
D.~Hynds$^{32}$,
P.~Ibis$^{15}$,
M.~Idzik$^{34}$,
D.~Ilin$^{38}$,
P.~Ilten$^{65}$,
A.~Inglessi$^{38}$,
A.~Ishteev$^{83}$,
K.~Ivshin$^{38}$,
R.~Jacobsson$^{48}$,
S.~Jakobsen$^{48}$,
E.~Jans$^{32}$,
B.K.~Jashal$^{47}$,
A.~Jawahery$^{66}$,
V.~Jevtic$^{15}$,
M.~Jezabek$^{35}$,
F.~Jiang$^{3}$,
M.~John$^{63}$,
D.~Johnson$^{48}$,
C.R.~Jones$^{55}$,
T.P.~Jones$^{56}$,
B.~Jost$^{48}$,
N.~Jurik$^{48}$,
S.~Kandybei$^{51}$,
Y.~Kang$^{3}$,
M.~Karacson$^{48}$,
M.~Karpov$^{82}$,
F.~Keizer$^{48}$,
M.~Kenzie$^{56}$,
T.~Ketel$^{33}$,
B.~Khanji$^{15}$,
A.~Kharisova$^{84}$,
S.~Kholodenko$^{44}$,
T.~Kirn$^{14}$,
V.S.~Kirsebom$^{49}$,
O.~Kitouni$^{64}$,
S.~Klaver$^{32}$,
K.~Klimaszewski$^{36}$,
S.~Koliiev$^{52}$,
A.~Kondybayeva$^{83}$,
A.~Konoplyannikov$^{41}$,
P.~Kopciewicz$^{34}$,
R.~Kopecna$^{17}$,
P.~Koppenburg$^{32}$,
M.~Korolev$^{40}$,
I.~Kostiuk$^{32,52}$,
O.~Kot$^{52}$,
S.~Kotriakhova$^{21,38}$,
P.~Kravchenko$^{38}$,
L.~Kravchuk$^{39}$,
R.D.~Krawczyk$^{48}$,
M.~Kreps$^{56}$,
F.~Kress$^{61}$,
S.~Kretzschmar$^{14}$,
P.~Krokovny$^{43,v}$,
W.~Krupa$^{34}$,
W.~Krzemien$^{36}$,
W.~Kucewicz$^{35,t}$,
M.~Kucharczyk$^{35}$,
V.~Kudryavtsev$^{43,v}$,
H.S.~Kuindersma$^{32,33}$,
G.J.~Kunde$^{67}$,
T.~Kvaratskheliya$^{41}$,
D.~Lacarrere$^{48}$,
G.~Lafferty$^{62}$,
A.~Lai$^{27}$,
A.~Lampis$^{27}$,
D.~Lancierini$^{50}$,
J.J.~Lane$^{62}$,
R.~Lane$^{54}$,
G.~Lanfranchi$^{23}$,
C.~Langenbruch$^{14}$,
J.~Langer$^{15}$,
O.~Lantwin$^{50}$,
T.~Latham$^{56}$,
F.~Lazzari$^{29,q}$,
R.~Le~Gac$^{10}$,
S.H.~Lee$^{86}$,
R.~Lef{\`e}vre$^{9}$,
A.~Leflat$^{40}$,
S.~Legotin$^{83}$,
O.~Leroy$^{10}$,
T.~Lesiak$^{35}$,
B.~Leverington$^{17}$,
H.~Li$^{72}$,
L.~Li$^{63}$,
P.~Li$^{17}$,
S.~Li$^{7}$,
Y.~Li$^{4}$,
Y.~Li$^{4}$,
Z.~Li$^{68}$,
X.~Liang$^{68}$,
T.~Lin$^{61}$,
R.~Lindner$^{48}$,
V.~Lisovskyi$^{15}$,
R.~Litvinov$^{27}$,
G.~Liu$^{72}$,
H.~Liu$^{6}$,
S.~Liu$^{4}$,
A.~Loi$^{27}$,
J.~Lomba~Castro$^{46}$,
I.~Longstaff$^{59}$,
J.H.~Lopes$^{2}$,
G.H.~Lovell$^{55}$,
Y.~Lu$^{4}$,
D.~Lucchesi$^{28,l}$,
S.~Luchuk$^{39}$,
M.~Lucio~Martinez$^{32}$,
V.~Lukashenko$^{32}$,
Y.~Luo$^{3}$,
A.~Lupato$^{62}$,
E.~Luppi$^{21,f}$,
O.~Lupton$^{56}$,
A.~Lusiani$^{29,m}$,
X.~Lyu$^{6}$,
L.~Ma$^{4}$,
R.~Ma$^{6}$,
S.~Maccolini$^{20,d}$,
F.~Machefert$^{11}$,
F.~Maciuc$^{37}$,
V.~Macko$^{49}$,
P.~Mackowiak$^{15}$,
S.~Maddrell-Mander$^{54}$,
O.~Madejczyk$^{34}$,
L.R.~Madhan~Mohan$^{54}$,
O.~Maev$^{38}$,
A.~Maevskiy$^{82}$,
D.~Maisuzenko$^{38}$,
M.W.~Majewski$^{34}$,
J.J.~Malczewski$^{35}$,
S.~Malde$^{63}$,
B.~Malecki$^{48}$,
A.~Malinin$^{81}$,
T.~Maltsev$^{43,v}$,
H.~Malygina$^{17}$,
G.~Manca$^{27,e}$,
G.~Mancinelli$^{10}$,
D.~Manuzzi$^{20,d}$,
D.~Marangotto$^{25,i}$,
J.~Maratas$^{9,s}$,
J.F.~Marchand$^{8}$,
U.~Marconi$^{20}$,
S.~Mariani$^{22,g}$,
C.~Marin~Benito$^{48}$,
M.~Marinangeli$^{49}$,
J.~Marks$^{17}$,
A.M.~Marshall$^{54}$,
P.J.~Marshall$^{60}$,
G.~Martellotti$^{30}$,
L.~Martinazzoli$^{48,j}$,
M.~Martinelli$^{26,j}$,
D.~Martinez~Santos$^{46}$,
F.~Martinez~Vidal$^{47}$,
A.~Massafferri$^{1}$,
M.~Materok$^{14}$,
R.~Matev$^{48}$,
A.~Mathad$^{50}$,
Z.~Mathe$^{48}$,
V.~Matiunin$^{41}$,
C.~Matteuzzi$^{26}$,
K.R.~Mattioli$^{86}$,
A.~Mauri$^{32}$,
E.~Maurice$^{12}$,
J.~Mauricio$^{45}$,
M.~Mazurek$^{48}$,
M.~McCann$^{61}$,
L.~Mcconnell$^{18}$,
T.H.~Mcgrath$^{62}$,
A.~McNab$^{62}$,
R.~McNulty$^{18}$,
J.V.~Mead$^{60}$,
B.~Meadows$^{65}$,
G.~Meier$^{15}$,
N.~Meinert$^{76}$,
D.~Melnychuk$^{36}$,
S.~Meloni$^{26,j}$,
M.~Merk$^{32,80}$,
A.~Merli$^{25}$,
L.~Meyer~Garcia$^{2}$,
M.~Mikhasenko$^{48}$,
D.A.~Milanes$^{74}$,
E.~Millard$^{56}$,
M.~Milovanovic$^{48}$,
M.-N.~Minard$^{8}$,
A.~Minotti$^{21}$,
L.~Minzoni$^{21,f}$,
S.E.~Mitchell$^{58}$,
B.~Mitreska$^{62}$,
D.S.~Mitzel$^{48}$,
A.~M{\"o}dden~$^{15}$,
R.A.~Mohammed$^{63}$,
R.D.~Moise$^{61}$,
T.~Momb{\"a}cher$^{46}$,
I.A.~Monroy$^{74}$,
S.~Monteil$^{9}$,
M.~Morandin$^{28}$,
G.~Morello$^{23}$,
M.J.~Morello$^{29,m}$,
J.~Moron$^{34}$,
A.B.~Morris$^{75}$,
A.G.~Morris$^{56}$,
R.~Mountain$^{68}$,
H.~Mu$^{3}$,
F.~Muheim$^{58,48}$,
M.~Mulder$^{48}$,
D.~M{\"u}ller$^{48}$,
K.~M{\"u}ller$^{50}$,
C.H.~Murphy$^{63}$,
D.~Murray$^{62}$,
P.~Muzzetto$^{27,48}$,
P.~Naik$^{54}$,
T.~Nakada$^{49}$,
R.~Nandakumar$^{57}$,
T.~Nanut$^{49}$,
I.~Nasteva$^{2}$,
M.~Needham$^{58}$,
I.~Neri$^{21}$,
N.~Neri$^{25,i}$,
S.~Neubert$^{75}$,
N.~Neufeld$^{48}$,
R.~Newcombe$^{61}$,
T.D.~Nguyen$^{49}$,
C.~Nguyen-Mau$^{49,x}$,
E.M.~Niel$^{11}$,
S.~Nieswand$^{14}$,
N.~Nikitin$^{40}$,
N.S.~Nolte$^{64}$,
C.~Normand$^{8}$,
C.~Nunez$^{86}$,
A.~Oblakowska-Mucha$^{34}$,
V.~Obraztsov$^{44}$,
D.P.~O'Hanlon$^{54}$,
R.~Oldeman$^{27,e}$,
M.E.~Olivares$^{68}$,
C.J.G.~Onderwater$^{79}$,
R.H.~O'neil$^{58}$,
A.~Ossowska$^{35}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{41}$,
P.~Owen$^{50}$,
A.~Oyanguren$^{47}$,
B.~Pagare$^{56}$,
P.R.~Pais$^{48}$,
T.~Pajero$^{63}$,
A.~Palano$^{19}$,
M.~Palutan$^{23}$,
Y.~Pan$^{62}$,
G.~Panshin$^{84}$,
A.~Papanestis$^{57}$,
M.~Pappagallo$^{19,c}$,
L.L.~Pappalardo$^{21,f}$,
C.~Pappenheimer$^{65}$,
W.~Parker$^{66}$,
C.~Parkes$^{62}$,
C.J.~Parkinson$^{46}$,
B.~Passalacqua$^{21}$,
G.~Passaleva$^{22}$,
A.~Pastore$^{19}$,
M.~Patel$^{61}$,
C.~Patrignani$^{20,d}$,
C.J.~Pawley$^{80}$,
A.~Pearce$^{48}$,
A.~Pellegrino$^{32}$,
M.~Pepe~Altarelli$^{48}$,
S.~Perazzini$^{20}$,
D.~Pereima$^{41}$,
P.~Perret$^{9}$,
M.~Petric$^{59,48}$,
K.~Petridis$^{54}$,
A.~Petrolini$^{24,h}$,
A.~Petrov$^{81}$,
S.~Petrucci$^{58}$,
M.~Petruzzo$^{25}$,
T.T.H.~Pham$^{68}$,
A.~Philippov$^{42}$,
L.~Pica$^{29,m}$,
M.~Piccini$^{78}$,
B.~Pietrzyk$^{8}$,
G.~Pietrzyk$^{49}$,
M.~Pili$^{63}$,
D.~Pinci$^{30}$,
F.~Pisani$^{48}$,
Resmi ~P.K$^{10}$,
V.~Placinta$^{37}$,
J.~Plews$^{53}$,
M.~Plo~Casasus$^{46}$,
F.~Polci$^{13}$,
M.~Poli~Lener$^{23}$,
M.~Poliakova$^{68}$,
A.~Poluektov$^{10}$,
N.~Polukhina$^{83,u}$,
I.~Polyakov$^{68}$,
E.~Polycarpo$^{2}$,
G.J.~Pomery$^{54}$,
S.~Ponce$^{48}$,
D.~Popov$^{6,48}$,
S.~Popov$^{42}$,
S.~Poslavskii$^{44}$,
K.~Prasanth$^{35}$,
L.~Promberger$^{48}$,
C.~Prouve$^{46}$,
V.~Pugatch$^{52}$,
H.~Pullen$^{63}$,
G.~Punzi$^{29,n}$,
H.~Qi$^{3}$,
W.~Qian$^{6}$,
J.~Qin$^{6}$,
N.~Qin$^{3}$,
R.~Quagliani$^{13}$,
B.~Quintana$^{8}$,
N.V.~Raab$^{18}$,
R.I.~Rabadan~Trejo$^{10}$,
B.~Rachwal$^{34}$,
J.H.~Rademacker$^{54}$,
M.~Rama$^{29}$,
M.~Ramos~Pernas$^{56}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{42,82}$,
G.~Raven$^{33}$,
M.~Reboud$^{8}$,
F.~Redi$^{49}$,
F.~Reiss$^{62}$,
C.~Remon~Alepuz$^{47}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{63}$,
R.~Ribatti$^{29}$,
S.~Ricciardi$^{57}$,
K.~Rinnert$^{60}$,
P.~Robbe$^{11}$,
G.~Robertson$^{58}$,
A.B.~Rodrigues$^{49}$,
E.~Rodrigues$^{60}$,
J.A.~Rodriguez~Lopez$^{74}$,
A.~Rollings$^{63}$,
P.~Roloff$^{48}$,
V.~Romanovskiy$^{44}$,
M.~Romero~Lamas$^{46}$,
A.~Romero~Vidal$^{46}$,
J.D.~Roth$^{86}$,
M.~Rotondo$^{23}$,
M.S.~Rudolph$^{68}$,
T.~Ruf$^{48}$,
J.~Ruiz~Vidal$^{47}$,
A.~Ryzhikov$^{82}$,
J.~Ryzka$^{34}$,
J.J.~Saborido~Silva$^{46}$,
N.~Sagidova$^{38}$,
N.~Sahoo$^{56}$,
B.~Saitta$^{27,e}$,
M.~Salomoni$^{48}$,
D.~Sanchez~Gonzalo$^{45}$,
C.~Sanchez~Gras$^{32}$,
R.~Santacesaria$^{30}$,
C.~Santamarina~Rios$^{46}$,
M.~Santimaria$^{23}$,
E.~Santovetti$^{31,p}$,
D.~Saranin$^{83}$,
G.~Sarpis$^{59}$,
M.~Sarpis$^{75}$,
A.~Sarti$^{30}$,
C.~Satriano$^{30,o}$,
A.~Satta$^{31}$,
M.~Saur$^{15}$,
D.~Savrina$^{41,40}$,
H.~Sazak$^{9}$,
L.G.~Scantlebury~Smead$^{63}$,
A.~Scarabotto$^{13}$,
S.~Schael$^{14}$,
M.~Schiller$^{59}$,
H.~Schindler$^{48}$,
M.~Schmelling$^{16}$,
B.~Schmidt$^{48}$,
O.~Schneider$^{49}$,
A.~Schopper$^{48}$,
M.~Schubiger$^{32}$,
S.~Schulte$^{49}$,
M.H.~Schune$^{11}$,
R.~Schwemmer$^{48}$,
B.~Sciascia$^{23}$,
S.~Sellam$^{46}$,
A.~Semennikov$^{41}$,
M.~Senghi~Soares$^{33}$,
A.~Sergi$^{24}$,
N.~Serra$^{50}$,
L.~Sestini$^{28}$,
A.~Seuthe$^{15}$,
P.~Seyfert$^{48}$,
Y.~Shang$^{5}$,
D.M.~Shangase$^{86}$,
M.~Shapkin$^{44}$,
I.~Shchemerov$^{83}$,
L.~Shchutska$^{49}$,
T.~Shears$^{60}$,
L.~Shekhtman$^{43,v}$,
Z.~Shen$^{5}$,
V.~Shevchenko$^{81}$,
E.B.~Shields$^{26,j}$,
E.~Shmanin$^{83}$,
J.D.~Shupperd$^{68}$,
B.G.~Siddi$^{21}$,
R.~Silva~Coutinho$^{50}$,
G.~Simi$^{28}$,
S.~Simone$^{19,c}$,
N.~Skidmore$^{62}$,
T.~Skwarnicki$^{68}$,
M.W.~Slater$^{53}$,
I.~Slazyk$^{21,f}$,
J.C.~Smallwood$^{63}$,
J.G.~Smeaton$^{55}$,
A.~Smetkina$^{41}$,
E.~Smith$^{14}$,
M.~Smith$^{61}$,
A.~Snoch$^{32}$,
M.~Soares$^{20}$,
L.~Soares~Lavra$^{9}$,
M.D.~Sokoloff$^{65}$,
F.J.P.~Soler$^{59}$,
A.~Solovev$^{38}$,
I.~Solovyev$^{38}$,
F.L.~Souza~De~Almeida$^{2}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{15}$,
E.~Spadaro~Norella$^{25,i}$,
P.~Spradlin$^{59}$,
F.~Stagni$^{48}$,
M.~Stahl$^{65}$,
S.~Stahl$^{48}$,
P.~Stefko$^{49}$,
O.~Steinkamp$^{50,83}$,
O.~Stenyakin$^{44}$,
H.~Stevens$^{15}$,
S.~Stone$^{68}$,
M.E.~Stramaglia$^{49}$,
M.~Straticiuc$^{37}$,
D.~Strekalina$^{83}$,
F.~Suljik$^{63}$,
J.~Sun$^{27}$,
L.~Sun$^{73}$,
Y.~Sun$^{66}$,
P.~Svihra$^{62}$,
P.N.~Swallow$^{53}$,
K.~Swientek$^{34}$,
A.~Szabelski$^{36}$,
T.~Szumlak$^{34}$,
M.~Szymanski$^{48}$,
S.~Taneja$^{62}$,
A.R.~Tanner$^{54}$,
A.~Terentev$^{83}$,
F.~Teubert$^{48}$,
E.~Thomas$^{48}$,
K.A.~Thomson$^{60}$,
V.~Tisserand$^{9}$,
S.~T'Jampens$^{8}$,
M.~Tobin$^{4}$,
L.~Tomassetti$^{21,f}$,
D.~Torres~Machado$^{1}$,
D.Y.~Tou$^{13}$,
M.T.~Tran$^{49}$,
E.~Trifonova$^{83}$,
C.~Trippl$^{49}$,
G.~Tuci$^{29,n}$,
A.~Tully$^{49}$,
N.~Tuning$^{32,48}$,
A.~Ukleja$^{36}$,
D.J.~Unverzagt$^{17}$,
E.~Ursov$^{83}$,
A.~Usachov$^{32}$,
A.~Ustyuzhanin$^{42,82}$,
U.~Uwer$^{17}$,
A.~Vagner$^{84}$,
V.~Vagnoni$^{20}$,
A.~Valassi$^{48}$,
G.~Valenti$^{20}$,
N.~Valls~Canudas$^{85}$,
M.~van~Beuzekom$^{32}$,
M.~Van~Dijk$^{49}$,
E.~van~Herwijnen$^{83}$,
C.B.~Van~Hulse$^{18}$,
M.~van~Veghel$^{79}$,
R.~Vazquez~Gomez$^{46}$,
P.~Vazquez~Regueiro$^{46}$,
C.~V{\'a}zquez~Sierra$^{48}$,
S.~Vecchi$^{21}$,
J.J.~Velthuis$^{54}$,
M.~Veltri$^{22,r}$,
A.~Venkateswaran$^{68}$,
M.~Veronesi$^{32}$,
M.~Vesterinen$^{56}$,
D.~~Vieira$^{65}$,
M.~Vieites~Diaz$^{49}$,
H.~Viemann$^{76}$,
X.~Vilasis-Cardona$^{85}$,
E.~Vilella~Figueras$^{60}$,
A.~Villa$^{20}$,
P.~Vincent$^{13}$,
D.~Vom~Bruch$^{10}$,
A.~Vorobyev$^{38}$,
V.~Vorobyev$^{43,v}$,
N.~Voropaev$^{38}$,
K.~Vos$^{80}$,
R.~Waldi$^{17}$,
J.~Walsh$^{29}$,
C.~Wang$^{17}$,
J.~Wang$^{5}$,
J.~Wang$^{4}$,
J.~Wang$^{3}$,
J.~Wang$^{73}$,
M.~Wang$^{3}$,
R.~Wang$^{54}$,
Y.~Wang$^{7}$,
Z.~Wang$^{50}$,
Z.~Wang$^{3}$,
H.M.~Wark$^{60}$,
N.K.~Watson$^{53}$,
S.G.~Weber$^{13}$,
D.~Websdale$^{61}$,
C.~Weisser$^{64}$,
B.D.C.~Westhenry$^{54}$,
D.J.~White$^{62}$,
M.~Whitehead$^{54}$,
D.~Wiedner$^{15}$,
G.~Wilkinson$^{63}$,
M.~Wilkinson$^{68}$,
I.~Williams$^{55}$,
M.~Williams$^{64}$,
M.R.J.~Williams$^{58}$,
F.F.~Wilson$^{57}$,
W.~Wislicki$^{36}$,
M.~Witek$^{35}$,
L.~Witola$^{17}$,
G.~Wormser$^{11}$,
S.A.~Wotton$^{55}$,
H.~Wu$^{68}$,
K.~Wyllie$^{48}$,
Z.~Xiang$^{6}$,
D.~Xiao$^{7}$,
Y.~Xie$^{7}$,
A.~Xu$^{5}$,
J.~Xu$^{6}$,
L.~Xu$^{3}$,
M.~Xu$^{7}$,
Q.~Xu$^{6}$,
Z.~Xu$^{5}$,
Z.~Xu$^{6}$,
D.~Yang$^{3}$,
S.~Yang$^{6}$,
Y.~Yang$^{6}$,
Z.~Yang$^{3}$,
Z.~Yang$^{66}$,
Y.~Yao$^{68}$,
L.E.~Yeomans$^{60}$,
H.~Yin$^{7}$,
J.~Yu$^{71}$,
X.~Yuan$^{68}$,
O.~Yushchenko$^{44}$,
E.~Zaffaroni$^{49}$,
M.~Zavertyaev$^{16,u}$,
M.~Zdybal$^{35}$,
O.~Zenaiev$^{48}$,
M.~Zeng$^{3}$,
D.~Zhang$^{7}$,
L.~Zhang$^{3}$,
S.~Zhang$^{5}$,
Y.~Zhang$^{5}$,
Y.~Zhang$^{63}$,
A.~Zharkova$^{83}$,
A.~Zhelezov$^{17}$,
Y.~Zheng$^{6}$,
X.~Zhou$^{6}$,
Y.~Zhou$^{6}$,
X.~Zhu$^{3}$,
Z.~Zhu$^{6}$,
V.~Zhukov$^{14,40}$,
J.B.~Zonneveld$^{58}$,
Q.~Zou$^{4}$,
S.~Zucchelli$^{20,d}$,
D.~Zuliani$^{28}$,
G.~Zunica$^{62}$.\bigskip

{\footnotesize \it

$^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{4}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{5}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{6}$University of Chinese Academy of Sciences, Beijing, China\\
$^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{8}$Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{12}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{13}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{14}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{15}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{16}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{17}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{18}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{19}$INFN Sezione di Bari, Bari, Italy\\
$^{20}$INFN Sezione di Bologna, Bologna, Italy\\
$^{21}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{22}$INFN Sezione di Firenze, Firenze, Italy\\
$^{23}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{24}$INFN Sezione di Genova, Genova, Italy\\
$^{25}$INFN Sezione di Milano, Milano, Italy\\
$^{26}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{27}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{28}$Universita degli Studi di Padova, Universita e INFN, Padova, Padova, Italy\\
$^{29}$INFN Sezione di Pisa, Pisa, Italy\\
$^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{31}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{32}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{33}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{35}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{36}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{37}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{38}$Petersburg Nuclear Physics Institute NRC Kurchatov Institute (PNPI NRC KI), Gatchina, Russia\\
$^{39}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$^{40}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$^{41}$Institute of Theoretical and Experimental Physics NRC Kurchatov Institute (ITEP NRC KI), Moscow, Russia\\
$^{42}$Yandex School of Data Analysis, Moscow, Russia\\
$^{43}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$^{44}$Institute for High Energy Physics NRC Kurchatov Institute (IHEP NRC KI), Protvino, Russia, Protvino, Russia\\
$^{45}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{46}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{47}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{48}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{49}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{50}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{51}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{52}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{53}$University of Birmingham, Birmingham, United Kingdom\\
$^{54}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{55}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{56}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{57}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{58}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{59}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{60}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{61}$Imperial College London, London, United Kingdom\\
$^{62}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{63}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{64}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{65}$University of Cincinnati, Cincinnati, OH, United States\\
$^{66}$University of Maryland, College Park, MD, United States\\
$^{67}$Los Alamos National Laboratory (LANL), Los Alamos, United States\\
$^{68}$Syracuse University, Syracuse, NY, United States\\
$^{69}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{56}$\\
$^{70}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$^{71}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$^{72}$Guangdong Provencial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$^{73}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$^{74}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{13}$\\
$^{75}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{17}$\\
$^{76}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{17}$\\
$^{77}$Eotvos Lorand University, Budapest, Hungary, associated to $^{48}$\\
$^{78}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{21}$\\
$^{79}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{32}$\\
$^{80}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{32}$\\
$^{81}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{41}$\\
$^{82}$National Research University Higher School of Economics, Moscow, Russia, associated to $^{42}$\\
$^{83}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{41}$\\
$^{84}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{41}$\\
$^{85}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{45}$\\
$^{86}$University of Michigan, Ann Arbor, United States, associated to $^{68}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{c}$Universit{\`a} di Bari, Bari, Italy\\
$^{d}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{e}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{f}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{g}$Universit{\`a} di Firenze, Firenze, Italy\\
$^{h}$Universit{\`a} di Genova, Genova, Italy\\
$^{i}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{j}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{k}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{l}$Universit{\`a} di Padova, Padova, Italy\\
$^{m}$Scuola Normale Superiore, Pisa, Italy\\
$^{n}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{o}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{p}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{q}$Universit{\`a} di Siena, Siena, Italy\\
$^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{s}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$^{t}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
$^{u}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$^{v}$Novosibirsk State University, Novosibirsk, Russia\\
$^{w}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden\\
$^{x}$Hanoi University of Science, Hanoi, Vietnam\\
\medskip
}
\end{flushleft}


==> LHCb_Authorship_DD-MMM-20YY.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = LHCb-PAPER-2021-011

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> acknowledgements.tex <==
\section*{Acknowledgements}
\noindent 
We express our gratitude to our colleagues in the CERN
accelerator departments for the excellent performance of the LHC. We
thank the technical and administrative staff at the LHCb
institutes.
We acknowledge support from CERN and from the national agencies:
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 (France); 
BMBF, DFG and MPG (Germany); 
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MEN/IFA (Romania); 
MSHE (Russia); 
MICINN (Spain); 
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).
We acknowledge the computing resources that are provided by CERN, IN2P3
(France), KIT and DESY (Germany), INFN (Italy), SURF (Netherlands),
PIC (Spain), GridPP (United Kingdom), RRCKI and Yandex
LLC (Russia), CSCS (Switzerland), IFIN-HH (Romania), CBPF (Brazil),
PL-GRID (Poland) and NERSC (USA).
We are indebted to the communities behind the multiple open-source
software packages on which we depend.
Individual groups or members have received support from
ARC and ARDC (Australia);
AvH Foundation (Germany);
EPLANET, Marie Sk\l{}odowska-Curie Actions and ERC (European Union);
A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP, 
Fundamental Research Funds for the Central Universities, 
and Sci. \& Tech. Program of Guangzhou (China);
%Key Research Program of Frontier Sciences of CAS, CAS PIFI,
%Thousand Talents Program, and Sci. \& Tech. Program of Guangzhou (China);
RFBR, RSF and Yandex LLC (Russia);
GVA, XuntaGal and GENCAT (Spain);
the Leverhulme Trust, the Royal Society
 and UKRI (United Kingdom).




==> body.tex <==
\section{Introduction}%
\label{sec:introduction}

The quark model~\cite{GellMann:1964nj,Zweig:1981pd,Zweig:1964jf} 
describes a doubly charmed baryon as a system of two bound charm quarks and a light quark (\uquark, \dquark or \squark).
There are three doubly charmed, weakly decaying states expected: a \Xicc isodoublet $(ccu,ccd)$ and an
\Omegacc isosinglet $(ccs)$, each with spin-parity $J^{P} = 1/2^{+}$. Theoretical models~\cite{Fleck:1989mb,Berezhnoy:1998aa, Ebert:2002ig, Chang:2006eu} predict that the light quark moves with a large relative velocity with respect to the bound ($cc$)-diquark inside the baryon and experiences a short-range of QCD potential. 

The \Xiccpp baryon with mass $3620.6 \pm 1.6$\mevcc was first observed by the LHCb collaboration in the \Lc\Km\pip\pip decay\footnote{Inclusion of charge-conjugated processes is implied throughout this paper.}~\cite{LHCb-PAPER-2017-018}, and confirmed in the $\Xicp\pip$ decay~\cite{LHCb-PAPER-2018-026}. The search for \Xiccp via its decay to \Lc\Km\pip was updated recently by the LHCb collaboration, and no significant signal was found~\cite{LHCb-PAPER-2019-029}. The \Omegacc mass is predicted to be in the range  $3.6-3.9\gevcc$~\cite{Ebert:2002pd,Gershtein:2000pd,Ebert:1997pc,Roncaglia1:1995pd,Roncaglia2:1995pd,Korner:1994np,Narodetskii:2001hep,Zachary:2014pd} and its lifetime is predicted to be $75-180\fs$~\cite{Haiyang:2018pd,hsi2008lifetime, Ebert:2002ig, guberina1999inclusive,Karliner:2014gca,Kiselev:1998sy,Kiselev:2001fw}. 
Due to destructive Pauli interference~\cite{Haiyang:2018pd}, the \Xiccpp and \Omegacc baryons have a larger lifetime than that of the \Xiccp baryon which is shortened by the contribution from 
$W$ boson exchange between the charm and down quarks. In proton-proton ($pp$) collisions at a centre-of-mass energy of 13\tev, the production cross-section of the doubly charmed baryons is predicted to be within the range of $60-1800\nb$~\cite{Berezhnoy:1998aa,Kiselev:2001fw,Ma:2003zk,Chang:2006xp,Chang:2006eu,Zhang:2011hi,Chang:2005bf}, which is between $10^{-4}$ and $10^{-3}$ times that of the total charm quark production~\cite{Kiselev:2001fw}. 
The production cross-section of the \Omegacc baryon is expected to be about 1/3 of those of the
\Xiccp and \Xiccpp baryons due to the presence of an $\squark$ quark~\cite{Berezhnoy:2018pd}. A discovery of the \Omegacc baryon would validate a prediction of the Standard Model. Besides, the study of doubly charmed baryons will also 
deepen our understanding of perturbative and non-perturbative QCD dynamics.


\begin{figure}[!htp]
  \centering
  \includegraphics[width=0.55\linewidth]{Figs/Fig1.pdf}
  \caption{Example Feynman diagram for the $\Omegacc\to\Xicp\Km\pip$ decay.}
  \label{fig:feynman1}
\end{figure}

In this paper, a search for the \Omegacc baryon via the $\Omegacc \to
\Xicp \Km \pip$ decay, which is predicted to have a relatively large branching fraction~\cite{Shi:2017dto,Jiang:2018}, is presented. The data are collected by the LHCb experiment in $pp$ collisions at a centre-of-mass energy of 13\tev in the period from 2016 to 2018. A possible Feynman diagram for this decay
is shown in Fig.~\ref{fig:feynman1}. 

In order to avoid experimenter's bias, the results of the analysis were not examined until the full procedure had been finalised.
Two different selections are developed: selection A is optimised to maximise the hypothetical signal sensitivity and selection B is optimised for the production ratio measurement. 
The analysis strategy is defined as follows:
\mbox{selection A} is first used to search for $\Omegacc$ signal   
and evaluate its significance as a function of $\Omegacc$ mass. 
If evidence for a signal with a global significance above 3 standard deviations after considering the look-elsewhere effect would be found, the mass would be measured and Selection B would be employed to measure the production cross-section of the \Omegacc baryon;
else, upper limits on the production ratio $R$ as a function of the \Omegacc mass for different lifetime hypotheses would be set. The production ratio $R$, relative to the $\Xiccpp \to \Lc\Km\pip\pip$ decay, is defined as
\begin{equation}
  \label{eq:RXicc}
  R \equiv \frac{\sigma(\Omegacc)\times\BF(\Omegacc \to
  \Xicp\Km\pip)\times\BF(\Xicp \to
  \proton\Km\pip)}{\sigma(\Xiccpp)\times\BF(\Xiccpp \to \Lc\Km\pip\pip)\times\BF(\Lc \to
  \proton\Km\pip)},
\end{equation}
where $\sigma$ is the baryon production cross-section and
$\mathcal{B}$ is the branching fraction of the corresponding decays. Both the $\Omegacc$ and $\Xiccpp$ baryons are required to be in the rapidity range of 2.0 to 4.5 and have  transverse momentum between 4 and 15 \gevc.

The production ratio is evaluated as
\begin{equation}
\label{eq:alphaN}
  R = \frac{\varepsilon_{\text{norm}}}{\varepsilon_{\text{sig}}}
                \frac{N_{\text{sig}}}{N_{\text{norm}}}
              \equiv \alpha N_{\text{sig}},
\end{equation}
where $\varepsilon_{\text{sig}}$ and $\varepsilon_{\text{norm}}$ 
refer to the efficiencies of the \Omegacc signal 
and the \Xiccpp normalisation decay mode, respectively,
$N_{\text{sig}}$ and $N_{\text{norm}}$ are the corresponding yields, and $\alpha$
is the single-event sensitivity. 
The lifetime of the \Omegacc baryon is unknown and strongly affects the selection efficiency,
hence upper limits on $R$
are quoted as a function of the \Omegacc baryon mass  
for a discrete set of lifetime hypotheses.


\section{Detector and simulation}%
\label{sec:Detector}

The \lhcb detector~\cite{LHCb-DP-2008-001,LHCb-DP-2014-002} is 
a single-arm forward
spectrometer covering the \mbox{pseudorapidity} range $2<\eta <5$,
designed for the study of particles containing \bquark or \cquark
quarks. The detector includes a high-precision tracking system
consisting of a silicon-strip vertex detector surrounding the $pp$
interaction region~\cite{LHCb-DP-2014-001},
a large-area silicon-strip detector located
upstream of a dipole magnet with a bending power of about
$4{\mathrm{\,Tm}}$, and three stations of silicon-strip detectors and straw
drift tubes~\cite{LHCb-DP-2013-003,LHCb-DP-2017-001}
placed downstream of the magnet.
The tracking system provides a measurement of the momentum, \ptot, of charged particles with
a relative uncertainty that varies from 0.5\% at low momentum to 1.0\% at 200\gevc.
The minimum distance of a track to a primary $pp$-collision vertex (PV), the impact parameter (IP), 
is measured with a resolution of $(15+29/\pt)\mum$,
where \pt is the component of the momentum transverse to the beam, in\,\gevc.
Different types of charged hadrons are distinguished using information
from two ring-imaging Cherenkov detectors\cite{LHCb-DP-2012-003}. 
The online event selection is performed by a trigger~\cite{LHCb-DP-2012-004}, 
which consists of a hardware stage, based on information from the calorimeter and muon
systems, followed by a software stage, which applies a full event
reconstruction.

Simulated samples are required to develop the event selection and
to estimate the detector acceptance and the
efficiency of the imposed selection requirements.
Simulated $pp$ collisions are generated using
\pythia~\cite{Sjostrand:2007gs,*Sjostrand:2006za} 
with a specific \lhcb configuration~\cite{LHCb-PROC-2010-056}.  
A dedicated generator, \genxicctwo~\cite{Chang:2009va},
is used to simulate the doubly charmed baryon production.
Decays of unstable particles
are described by \evtgen~\cite{Lange:2001uf}, in which final-state
radiation is generated using \photos~\cite{davidson2015photos}. The
interaction of the generated particles with the detector, and its response,
are implemented using the \geant
toolkit~\cite{Allison:2006ve, *Agostinelli:2002hh} as described in
Ref.~\cite{LHCb-PROC-2011-006}.
Unless otherwise stated,
simulated events are generated with an \Omegacc (\Xiccpp) mass of 3738\mevcc (3621\mevcc) 
and a lifetime of 160\fs (256\fs).


\section{Reconstruction and selection}%
\label{sec:reconstruction_and_selection}

The \Omegacc signal mode is reconstructed by combining a \Xicp candidate with kaon and pion candidates coming from the same vertex. The \Xicp candidates are firstly formed by combining three tracks originating from the same vertex, displaced with respect to the PV; at least one track is required to satisfy an inclusive software trigger based on a multivariate classifier~\cite{pmlr-v14-gulin11a, LHCb-PROC-2015-018}, and the three tracks must satisfy particle identification (PID) requirements to be compatible with a $\proton\Km\pip$ hypothesis. Then the \Xicp candidates with good vertex quality and invariant mass within the region of 2450 to 2486 \mevcc are combined with two extra tracks, identified as \Km and \pip , to reconstruct a \Omegacc candidate. The \Xicp mass region is defined as $2468\pm18 \mevcc$ where the mean value is the known \Xicp mass~\cite{PDG2020} and 
the width is corresponding to three
times the mass resolution.

To improve further the \Omegacc signal purity, a multivariate classifier based on a boosted decision tree (BDT)~\cite{Breiman,Hocker:2007ht,*TMVA4} is developed to suppress combinatorial background. 
The classifier is trained using simulated \Omegacc events as signal and wrong-sign $\Xicp\Km\pim$ combinations in data with mass 
in the interval 3600 to 4000\mevcc to represent background.

For \mbox{selection A}, no specific trigger requirement is applied. A multivariate selection is trained with two sets of variables which show good discrimination between \Omegacc signal and background. The first set contains variables related to the reconstructed \Omegacc candidates, including the \Omegacc decay vertex-fit quality, such as \chisqip, the pointing angle and the flight-distance \chisq. Here \chisqip is the difference in \chisq of the PV reconstructed with and without the \Omegacc candidate, the pointing angle is the three-dimensional angle between the \Omegacc
candidate momentum direction and the vector joining the PV and the reconstructed \Omegacc decay vertex, while the flight-distance \chisq is defined as the \chisq of the hypothesis that the decay vertex of the candidate coincides with its associated PV. The second set adds variables related to the decay products (\proton, \Km and \pip from the \Xicp decay, and \Km and \pip from the \Omegacc decay), including  momentum,  transverse momentum,  \chisqip and  PID variables.

The threshold of the multivariate output is determined by maximising 
the figure of merit $\varepsilon/\left(5/2 + \sqrt{N_B}\right)$~\cite{Punzi:2003bu}, where $\varepsilon$ is the estimated MVA selection efficiency, 
$5/2$ corresponds to 5 standard deviations in a Gaussian significance test, 
and $N_B$ is the expected number of background candidates
in the signal region, estimated with the wrong-sign $\Xicp\Km\pim$ combinations in the mass region of $\pm12.5\mevcc$ around the  \Omegacc mass of 3738\mevcc used in the simulation, taking into account the difference of the background level for the signal sample and the wrong-sign sample.


After the multivariate selection, events may still contain more than one \Omegacc candidate in the signal region although the probability to produce more than one \Omegacc is small. The reconstructed \Omegacc candidates could suffer from background from candidates reconstructed with clone tracks, i.e. reconstructed tracks sharing a large portion of their detector hits. Clone tracks could be included in a \Omegacc candidate, when one is used for the \pip candidate from the \Xicp decay and its clone for the \pip candidate from the \Omegacc decay. To avoid that, candidates with the angle between each pair of identically charged tracks smaller than 0.5~mrad are removed. The \Omegacc candidates could also be formed by the same five final tracks but with two tracks interchanged, \eg the \Km (\pip) candidate from the \Xicp decay is swapped with the \Km (\pip) candidate from the \Omegacc decay. In this case, only one  candidate is chosen randomly.



For \mbox{selection B},
the multivariate selection is similar to \mbox{selection A} except that the 
PID variables of the \Km and \pip candidates from the \Omegacc decay are not used in the training to ease the efficiency determination. Furthermore, an additional hardware trigger requirement is imposed on candidates for both the signal and the normalisation modes to minimise differences between data and simulation. 
The data sets are split into two disjoint subsamples. One subsample is triggered on signals associated with one of the reconstructed \Xicp candidates with high transverse energy deposits in the calorimeters (TOS), and the other is triggered on signals exclusively unrelated to the \Omegacc candidate (exTIS).

The reconstruction and selection requirements of the \Xiccpp normalisation mode are similar to those in the \Xiccp search~\cite{LHCb-PAPER-2019-029,LHCb-PAPER-2019-035}.
Both \Omegacc and \Xiccpp candidates are required to be in the fiducial region of
rapidity $2.0<y<4.5$ and transverse momentum $4<\pt<15\gevc$.


\section{Yield measurements}
\label{sec:yield}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.70\linewidth]{Figs/Fig2.pdf}
  \caption{Invariant mass $m(\Xicp\Km\pip)$ distribution of selected \Omegacc candidates from (black points) selection A, with (blue solid line) the fit with the largest local significance at the mass of 3876\mevcc superimposed.}
  \label{fig:fit_shape}
\end{figure}

After applying \mbox{selection A} to the full data sample,  
the invariant mass distribution $m(\Xicp\Km\pip)$ of selected $\Omegacc$ candidates is shown in Fig.~\ref{fig:fit_shape}. 
To improve the mass resolution, 
the variable 
 $m(\Xicp\Km\pip)$ is defined as the difference of the reconstructed mass of the \Omegacc and \Xicp candidates plus the known \Xicp mass~\cite{PDG2020}.
The $m(\Xicp\Km\pip)$ distribution is fitted with a sum of signal and background components, where the signal component is described by the sum of two Crystal Ball functions~\cite{Skwarnicki:1986xj} and the background component by a second-order Chebyshev function. The parameters of the signal shape are fixed from simulation, where the width is found to be around 5.5\mevcc. The parameters of background shape are obtained from a fit to the wrong-sign $\Xicp\Km\pim$ combinations. An unbinned maximum likelihood fit is performed with the peak position varied in steps of \\
2 \mevcc, and the largest signal contribution is found for an \Omegacc mass of 3876\mevcc. 


The local significance of the signal peak is quantified with a $p$-value, which is calculated as the likelihood ratio of the background plus signal hypothesis and the background-only hypothesis~\cite{Wilks:1938dza,Narsky:2000}.
The local $p$-value is plotted in Fig.~\ref{fig:pvalue} as a function of mass, $m(\Xicp\Km\pip)$, showing a dip around 3876\mevcc, which has the largest local significance, corresponding to $3.2$
standard deviations. The global significance is evaluated with pseudoexperiments, by taking into account the look-elsewhere effect~\cite{Gross:2010qma} in the mass range from 3600\mevcc to 4000\mevcc, and is estimated to be $1.8$ standard deviations.
As no excess above 3 standard deviations is observed,
upper limits on the production ratios are set by using \mbox{selection B}. The invariant mass distribution of \Omegacc candidates is shown in Fig.~\ref{fig:selectionB_fit} with the fit under the background-only hypothesis.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.7\linewidth]{Figs/Fig3.pdf}
  \caption{Local $p$-value at different $m(\Omegacc)$ values
  evaluated with the likelihood ratio test. Lines indicating one, two and three standard deviations ($\sigma$)  of local significance are also shown.}
  \label{fig:pvalue}
\end{figure}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.70\linewidth]{Figs/Fig4.pdf}
  \caption{Invariant mass $m(\Xicp\Km\pip)$ distribution of selected \Omegacc candidates (black points) with selection B, only background fit is shown.}
  \label{fig:selectionB_fit}
\end{figure}

The measured production ratio is a function of single-event sensitivity $\alpha$ and $N_{\text{sig}}$, as shown in Eq.~\ref{eq:alphaN}. The parameter $\alpha$ is calculated using the yield of the normalisation mode $N_{\text{norm}}$ multiplied by the efficiency ratio between the normalisation and signal modes, while $N_{\text{sig}}$ is extracted by fitting the data of the signal mode.

The $\Xiccpp$ yields, $N_{\text{norm}}$, are determined by performing an extended unbinned maximum likelihood fit to the invariant mass in the two trigger categories. The invariant mass distribution $m(\Lcp\Km\pip\pip)$ is defined as the difference of the reconstructed mass of the \Xiccpp and \Lc candidates plus the known \Lc mass~\cite{PDG2020}.
For illustration,
the $m(\Lc\Km\pip\pip)$ distributions for the 2018 data set
are shown in Fig.~\ref{fig:yield_xicc} together with  the associated fit projections. 
The mass shapes of the normalisation mode are a sum of a Gaussian function and a modified Gaussian function with power-law tails on both sides for signal and a second-order Chebyshev polynomial for background, which is the same as used in the \Xiccp search~\cite{LHCb-PAPER-2019-035}.
The \Xiccpp yields are summarised in Table~\ref{tab:yield_summary}, where the TOS refers to the trigger on signal and the exTIS refers to exclusive trigger independently of signal. 

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.98\linewidth]{Figs/Fig5.pdf}
  \caption{Distribution of invariant mass $m(\Lc\Km\pip\pip)$ for selected $\Xiccpp$ candidates in different categories:  (a)~triggered by one of the \Lcp decay products and (b)~triggered exclusively by particles unrelated to the \Xiccpp decay products, in the 2018 data set. The fit results are superimposed.}
  \label{fig:yield_xicc}
\end{figure}



\begin{table}[bt]
  \centering
  \caption{Signal yields for the $\Xiccpp\to\Lc\Km\pip\pip$ normalisation mode $N_{\text{norm}}$ for both trigger categories and different data-taking periods with the corresponding integrated luminosity $\mathcal{L}$. The uncertainties are statistical only.}
  \label{tab:yield_summary}
  \begin{tabular}{cccc}
    \toprule
    \multirow{2}*{Year} & \multirow{2}*{$\mathcal{L}$ $[\invfb]$} &\multicolumn{2}{c}{$N_{\text{norm}}$} \\ 
 \cline{3-4}
 ~ & ~ & \multirow{1.2}*{TOS} & \multirow{1.2}*{exTIS}\\
    \midrule
    2016&   1.7&  $126\pm21$   & $165\pm23$ \\
    2017&   1.6&  $145\pm21$   & $255\pm26$ \\
    2018&   2.1&  $164\pm21$  & $349\pm30$ \\
    \bottomrule
  \end{tabular}
\end{table}



\section{Efficiency ratio estimation}%
\label{sec:efficiency_ratio}
The efficiency ratio between the \Xiccpp mode and \Omegacc mode, defined as $\eps_{\rm norm}/\eps_{\rm sig}$, is determined from simulation,
where kinematic distributions are weighted to match those in data. 
The tracking and PID efficiencies for both normalisation and signal modes are corrected using calibration data samples~\cite{LHCb-DP-2013-002,LHCb-PUB-2016-021,LHCb-DP-2018-001}. 
The efficiency ratio of both trigger categories for different data-taking periods are summarised in Table~\ref{tab:eff_ratio}. Since there is an additional track in the \Xiccpp decay when compared to the \Omegacc decay, the reconstruction and selection efficiency of \Xiccpp candidates is significantly lower. The increase in the efficiency ratio for the 2017 and 2018 data is due to the optimisation of the \Xiccpp online selection, following the observation of the \Xiccpp baryon~\cite{LHCb-PAPER-2017-018}.

\begin{table}[tb]
  \centering
  \caption{Efficiency ratios $\eps_{\rm norm}/\eps_{\rm sig}$ between  normalisation and signal modes for both trigger categories for 
  different data-taking periods, where the TOS refers to the trigger on signal and the exTIS refers to exclusive trigger independently of signal. The uncertainties are statistical only.}
\label{tab:eff_ratio}
\begin{tabular}{ccc} 
\toprule 
\multirow{2}*{Year} & \multicolumn{2}{c}{$\eps_{\rm norm}/\eps_{\rm sig}$} \\ 
 \cline{2-3}
 ~ & \multirow{1.2}*{TOS} & \multirow{1.2}*{exTIS}\\
\midrule 
2016& 0.32 $\pm$ 0.03 & 0.28 $\pm$ 0.02\\ 
2017& 0.55 $\pm$ 0.03 & 0.71 $\pm$ 0.02\\ 
2018& 0.61 $\pm$ 0.04 & 0.69 $\pm$ 0.02\\ 
\bottomrule 
\end{tabular} 
\end{table}

In order to take into account the dependence of the selection efficiency upon the unknown value of the \Omegacc lifetime, simulated \Omegacc events
are weighted to reproduce different exponential decay time distributions corresponding to lifetimes of 40\fs, 80\fs, 120\fs, 160\fs , and 200\fs. This method is used to estimate the change in the efficiency. 
The single-event sensitivities are calculated by the ratio of \Xiccpp efficiency to the \Omegacc efficiency with different lifetime hypotheses, as shown in Tables~\ref{tab:alpha_TOS} and~\ref{tab:alpha_TIS}, for both trigger categories.

\begin{table}[tb]
  \centering
  \caption{Single-event sensitivity $\alpha(\Xiccpp)$ [$10^{-2}$] of the \Xiccpp normalisation mode triggered by one of the \Xicp (\Lcp) products for different lifetime hypotheses of the $\Omegacc$ baryon for different data-taking periods.
  The uncertainties are due to the limited size of the simulated samples
  and the statistical uncertainties on the measured \Xiccpp baryon yields.}
\label{tab:alpha_TOS}
\begin{tabular}{c rrrrr} 
\toprule 
\multirow{2}*{Year} & \multicolumn{5}{c}{$\alpha$ [$10^{-2}$]} \\ 
 \cline{2-6}
~ & \multirow{1.2}*{$\tau=40\fs$} & \multirow{1.2}*{$\tau=80\fs$} & \multirow{1.2}*{$\tau=120\fs$} & 
\multirow{1.2}*{$\tau=160\fs$} & \multirow{1.2}*{$\tau=200\fs$}\\ 
\midrule 
2016& 0.86 $\pm$ 0.17 & 0.46 $\pm$ 0.09 & 0.32 $\pm$ 0.06 & 0.25 $\pm$ 0.05 & 0.22 $\pm$ 0.04\\ 
2017& 1.29 $\pm$ 0.20 & 0.69 $\pm$ 0.11 & 0.48 $\pm$ 0.07 & 0.38 $\pm$ 0.06 & 0.33 $\pm$ 0.05\\ 
2018& 1.26 $\pm$ 0.18 & 0.67 $\pm$ 0.10 & 0.47 $\pm$ 0.07 & 0.37 $\pm$ 0.05 & 0.32 $\pm$ 0.05\\ 
\bottomrule 
\end{tabular} \end{table}


\begin{table}[!tb]
  \centering
  \caption{Single-event sensitivity $\alpha(\Xiccpp)$ [$10^{-2}$] of the \Xiccpp normalisation mode triggered exclusively by particles unrelated to the \Omegacc (\Xiccpp) decay products for different lifetime hypotheses of the $\Omegacc$ baryon in the different data-taking periods.
  The uncertainties are due to the limited size of the simulated samples
  and the statistical uncertainty on the measured \Xiccpp baryon yield.}
\label{tab:alpha_TIS}
\begin{tabular}{c rrrrr} 
\toprule 
\multirow{2}*{Year} & \multicolumn{5}{c}{$\alpha$ [$10^{-2}$]} \\ 
 \cline{2-6}
~ & \multirow{1.2}*{$\tau=40\fs$} & \multirow{1.2}*{$\tau=80\fs$} & \multirow{1.2}*{$\tau=120\fs$} & 
\multirow{1.2}*{$\tau=160\fs$} & \multirow{1.2}*{$\tau=200\fs$}\\
\midrule 
2016& 0.71 $\pm$ 0.11 & 0.35 $\pm$ 0.06 & 0.22 $\pm$ 0.04 & 0.17 $\pm$ 0.03 & 0.14 $\pm$ 0.02\\ 
2017& 1.16 $\pm$ 0.12 & 0.57 $\pm$ 0.06 & 0.37 $\pm$ 0.04 & 0.28 $\pm$ 0.03 & 0.23 $\pm$ 0.02\\ 
2018& 0.82 $\pm$ 0.08 & 0.41 $\pm$ 0.04 & 0.26 $\pm$ 0.02 & 0.20 $\pm$ 0.02 & 0.17 $\pm$ 0.02\\ 
\bottomrule 
\end{tabular} \end{table}


The \Omegacc mass is also unknown. To test the effects of different mass hypotheses,
two simulated samples are generated with $m(\Omegacc)=3638\mevcc$ and $m(\Omegacc)=3838\mevcc$.
These samples are used to weight the \pt distributions of final states in the \Omegacc decay
to match those in the other mass hypotheses, and the efficiency is recalculated with the weighted samples. When varying the \Omegacc mass, it is found that the efficiency is constant; therefore, the \Omegacc mass dependence is neglected in the evaluation of the single-event sensitivities.


\section{Systematic uncertainties}
The sources of systematic uncertainties on the production ratio $R$ are listed in Table~\ref{tab:sys_fit}, where individual sources are assumed to be independent and summed in quadrature to compute the total systematic uncertainty.  

The choice of the mass models used to fit the invariant mass distribution affects the normalisation yields and therefore affects the calculation of single-event sensitivities. The related systematic uncertainty is studied by using alternative functions to describe the signal and background shapes of the \Xiccpp mode.
The sum of two Gaussian functions is chosen as an alternative signal model and a second-order polynomial function is chosen to substitute the background model. The difference in the signal yields obtained by changing models is assigned as the systematic uncertainty.

The systematic uncertainty associated with the trigger efficiency is evaluated using a tag-and-probe method~\cite{LHCb-DP-2012-004}.
The size of the normalisation sample is insufficient to derive this systematic uncertainty. Instead, $b$-flavoured hadrons decaying with similar final-state topologies are used. 
For the TOS category, 
 \Lb\to\Lc\pip\pim\pim and
\Lb\to\Lc\pim candidates can be 
triggered by the energy deposit in the calorimeter by one of the \Lc decay products, which are similar to 
the $\Xiccpp \to \Lc\Km\pip\pip$ and $\Omegacc \to \Xicp\Km\pip$ decays. 
The efficiency ratio of these two \Lb modes is estimated and the difference of the ratio between data and simulation is assigned as a systematic uncertainty.  
For the exTIS category, the \Bc\to\jpsi\pip decay, which has two heavy-flavour particles ($b$- and $c$-hadrons) and is similar to the signal topology, is used to study the trigger efficiency with particle candidates that are independent and unrelated to the signal. The systematic uncertainty for the exTIS trigger category is assigned as the difference in the efficiency ratio of \Lb\to\Lc\pip\pim\pim mode to \Bc\to\jpsi\pip mode in data and in simulation.

The tracking efficiency is corrected with calibration data samples~\cite{LHCb-DP-2013-002}, and is affected by three sources of systematic uncertainties. 
First, the inaccuracy of the simulation in terms of detector occupancy, which is assigned as 1.5\% and 2.5\% for kaons and pions,  does not cancel in the ratio. An additional systematic uncertainty arises from the calibration method which provides a 0.8\% uncertainty per track~\cite{LHCb-DP-2013-002}. The third uncertainty is due to the limited size of the calibration samples and studied by pseudoexperiments. The tracking efficiency is corrected by the pseudoexperiments and the Gaussian width of the newly obtained distribution of the efficiency ratio is assigned as the systematic uncertainty.


The PID efficiency is determined in intervals of particle momentum, 
pseudorapidity and event multiplicity using calibration data samples. The corresponding sources of systematic uncertainty are due to the limited size of the calibration samples and the binning scheme used. To study their effects, a large number of pseudoexperiments are performed, and the binning scheme is varied. 


The \Xiccpp lifetime is measured with limited precision, $\ensuremath{256\,^{+24}_{-22}\,{\rm(stat)\,}\pm
14\,{\rm(syst)}\,\fs}$~\cite{LHCb-PAPER-2018-019}, which is propagated to the systematic uncertainty in the efficiency.

As the agreeemnt between data and simulation is limited, a difference of 5.0\% is found among different periods of data-taking, which is taken as systematic uncertainty.



 \begin{table}[tp]
    \centering
      \caption{Systematic uncertainties on the production ratio $R$.}
  \label{tab:sys_fit}
  \begin{tabular}{lr}
    \toprule
    Source & $R$~[\%] \\
    \midrule
    Fit model             & 3.5 \\
    Hardware trigger & 11.2  \\
    Tracking             & 2.7  \\
    PID   & 0.9  \\
    \Xiccpp lifetime &  12.0\\
    Simulation/data difference                  & 5.0 \\
       \midrule
    Total                        & 17.7 \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Results}%
\label{sec:results}
Upper limits on the production ratio $R$ are set with a simultaneous fit to the $m(\Xicp\Km\pip)$ distributions of different trigger categories for all the data sets from 2016 to 2018,
following the strategy described in Sec.~\ref{sec:yield} for the normalisation mode.
The upper limit values are calculated by setting different \Omegacc mass hypotheses in the fit within the $m(\Xicp\Km\pip)$ mass range from 3600 to 4000\mevcc with a step of 2\mevcc, for five different lifetime hypotheses, 40\fs, 80\fs, 120\fs, 160\fs , and 200\fs.

For each \Omegacc mass and lifetime hypothesis,  
the likelihood profile 
is determined as a function of $R$.
It is then convolved with a Gaussian distribution whose width is equal to the square root of the quadratic combination of the 
statistical and systematic uncertainties on the single-event sensitivity.
The upper limit at 95\% credibility level is defined as
the value of $R$ at which the integral of the profile likelihood equals 95\% of the total area. Figure~\ref{fig:mass_scan_tau_run2} 
shows the 95\% credibility level upper limits at different mass hypotheses for five different lifetimes. The upper limits on $R$ decrease when increasing the \Omegacc lifetime. Considering the whole explored mass range, the highest upper limit on $R$ is $0.11$  obtained under lifetime hypothesis of 40 fs while the lowest is $0.5 \times 10^{-2}$ obtained under lifetime hypothesis of 200 fs. 

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.70\linewidth]{Figs/Fig6.pdf}
  \caption{Upper limits on the production ratio $R$
  at 95\% credibility level as a function of $m(\Xicp\Km\pip)$ at
  $\sqrt{s}=13\tev$, 
  for five $\Omegacc$ lifetime hypotheses.}
  \label{fig:mass_scan_tau_run2}
\end{figure}


\section{Conclusion}%
\label{sec:conclusion}

A search for the \Omegacc baryon through the \Xicp\Km\pip decay is performed, using $pp$ collision data collected by the \lhcb experiment
from 2016 to 2018 at a centre-of-mass energy of 13\tev,  corresponding to an integrated luminosity of 5.4\invfb.
No significant signal is observed in the mass range of 3.6 to 4.0\gevcc.
Upper limits are set at $95\%$ credibility level
on the ratio of the \Omegacc production cross-section times
the branching fraction to that of the \Xiccpp baryon as a function of the \Omegacc mass and for different lifetime hypotheses, 
in the rapidity range of 2.0 to 4.5 and the transverse momentum range of 4 to 15\gevc.
The upper limits depend strongly on the mass and lifetime hypotheses of the \Omegacc, and vary from $1.1 \times 10^{-1}$ to $0.5 \times 10^{-2}$ for 40\fs to 200\fs, respectively.
Future searches by the \lhcb experiment with upgraded detector, improved trigger conditions, additional
$\Omegacc$ decay modes, and larger data samples will further increase the \Omegacc signal sensitivity. 





==> efficiency_variation.tex <==
\section{Variation of efficiency with mass and lifetime}%
\label{sec:variation_of_efficiency_with_mass_and_lifetime}

The efficiency depends strongly on the \Xiccp lifetime,
due to the use of lifetime-related variables in the selection.
Unfortunately, the prediction of \Xiccp lifetime has a large uncertainty.
Therefore, the upper limits vary under different lifetime hypotheses.
To take this effect into account, the efficiency is re-calculated under each
different lifetime hypothesis
%(a discrete set of $0\fs$, $40\fs$, $80\fs$, $120\fs$, and $160\fs$ is considered).
(a discrete set of $40\fs$, $80\fs$, $120\fs$, and $160\fs$ is considered).

For the non-zero lifetime hypotheses,
the MC sample generated with $\tau_0=333\fs$ is re-weighted
according to the TRUE decay time $t$ with the weight $w(t)$ defined as
$$ w(t) = \frac{\frac{1}{\tau}\text{exp}(-\frac{t}{\tau})}{\frac{1}{\tau_0}\text{exp}(-\frac{t}{\tau_0})}, $$
where $\tau$ is the lifetime hypothesis under study.
Hence, the efficiency for a given selection is
$$ \varepsilon = \frac{\sum_{\text{pass}} w_i}{\sum_{\text{before}} w_j}, $$
where the sum $i$ runs over the events that pass the selection and
$j$ runs over all the events before the selection.
For the zero lifetime hypothesis,
a dedicated MC sample generated with $\tau=0\fs$ is used to calculate the efficiency.
The results are summarised in Tables~\ref{tab:eff_vary_tau} and \ref{tab:eff_vary_tau_12},
and are visualised in Fig.~\ref{fig:eff_vary_tau}.
A roughly linear dependence of the efficiency on lifetime hypotheses is observed.

\begin{table}
  \centering
  \caption{Efficiencies at different lifetime hypotheses for 2016 data.}
  \label{tab:eff_vary_tau}
  \input{tables/Efficiency_VaryTau_16_dalitz}
\end{table}

\begin{table}
  \centering
  \caption{Efficiencies at different lifetime hypotheses for 2012 data.}
  \label{tab:eff_vary_tau_12}
  \input{tables/Efficiency_VaryTau_12_dalitz}
\end{table}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.49\linewidth]{efficiency/Efficiency_VaryTau.pdf}
  \includegraphics[width=0.49\linewidth]{efficiency/Efficiency_VaryTau_12.pdf}
  \caption{Efficiencies at different lifetime hypotheses for (left) 2016 and (right) 2012 data.}
  \label{fig:eff_vary_tau}
\end{figure}

The kinematics of final tracks depend on the mass of \Xiccp baryons.
Therefore, the efficiency may vary as a function of the mass.

To take into account this effect, a weighting procedure is developed.
Firstly, produce generator-level MC samples with different \Xiccp mass hypotheses
(here the values of $3518.7\mevcc$ and $3700.0\mevcc$ are considered.)
Secondly, re-weight the full-simulated sample (generated with $m_0 = 3621.4\mevcc$)
according to the generator-level \pt distributions of \Xiccp secondaries (\Lc, \Km and \pip from \Xiccp),
the efficiency is then re-calculated at each mass hypothesis.
The weights are acquired with the \texttt{GBReweightor} from the \texttt{hep\_ml} python module,
a reweightor algorithm based on ensemble of regression trees~\cite{gbreweight:1}.
%(\textcolor{red}{some citations here}).

The results are shown in Table~\ref{tab:eff_vary_mass} and visualized in Fig.~\ref{fig:eff_vary_mass}.
The dependence of the total efficiency on the \Xiccp mass hypotheses is weak in a wide range.
We tend to not include this effect when calculating the upper limits at different mass hypotheses.

\begin{table}[tb]
  \centering
  \caption{Efficiencies at different mass hypotheses.}
  \label{tab:eff_vary_mass}
  \input{tables/Efficiency_VaryMass}
\end{table}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.6\linewidth]{efficiency/Efficiency_VaryMass.pdf}
  \caption{Efficiency as a function of mass hypotheses.}
  \label{fig:eff_vary_mass}
\end{figure}



==> fixed-symbols-def.tex <==
%%% $Id: $
%%% ======================================================================
%%% Purpose: Private fixes, alternatives, and additions to standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes.  Private modifications by P. Spradlin.
%%% Maintainer : 
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
%%% BaBar macro used by BaBar.
%%%\def\babar  {\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em B\kern-0.1em{\smaller A\kern-0.2em R}}}

%% LHCb sub-detectors and sub-systems


%%% Upright (not slanted) Particles


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles


%% Leptons

%% Gauge bosons and scalars

%% Quarks

%% Light mesons

%% Heavy mesons

%% Onia

%% Baryons

%%% Missing cc versions of base macros
\def\DeltaOrDeltabar  {\kern 0.18em\optbar{\kern -0.18em \PDelta}{}\xspace}
\def\XiOrXibar        {\kern 0.18em\optbar{\kern -0.18em \PXi}{}\xspace}
\def\SigmaOrSigmabar  {\kern 0.18em\optbar{\kern -0.18em \PSigma}{}\xspace}
\def\OmegaOrOmegabar  {\kern 0.18em\optbar{\kern -0.18em \POmega}{}\xspace}


%%% Alternate and additional macros for charmed baryons
\def\Lcp          {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcm          {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Lcpm         {{\ensuremath{\LorLbar{}^{\pm}_\cquark}}\xspace}
\def\Xicp         {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicm         {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Xicpm        {{\ensuremath{\XiOrXibar{}_\cquark^{\pm}}}\xspace}
\def\Xiczbar      {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xiczorbar    {{\ensuremath{\XiOrXibar{}_\cquark^0}}\xspace}
\def\Sigmacpp     {{\ensuremath{\Sigmares^{++}_\cquark}}\xspace}
\def\Sigmacmm     {{\ensuremath{\Sigmaresbar{}^{--}_\cquark}}\xspace}
\def\Sigmacpmpm   {{\ensuremath{\SigmaOrSigmabar{}^{\pm\pm}_\cquark}}\xspace}
\def\Sigmacp      {{\ensuremath{\Sigmares^{+}_\cquark}}\xspace}
\def\Sigmacm      {{\ensuremath{\Sigmaresbar{}^{-}_\cquark}}\xspace}
\def\Sigmacpm     {{\ensuremath{\SigmaOrSigmabar{}^{\pm}_\cquark}}\xspace}
\def\Sigmacz      {{\ensuremath{\Sigmares^{0}_\cquark}}\xspace}
\def\Sigmaczbar   {{\ensuremath{\Sigmaresbar{}^{0}_\cquark}}\xspace}
\def\Sigmaczorbar {{\ensuremath{\SigmaOrSigmabar{}^{0}_\cquark}}\xspace}
\def\Xiccbare     {{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xiccpp       {{\ensuremath{\Xires^{++}_{\cquark\cquark}}}\xspace}
\def\Xiccmm       {{\ensuremath{\Xiresbar{}^{--}_{\cquark\cquark}}}\xspace}
\def\Xiccpmpm     {{\ensuremath{\XiOrXibar{}^{\pm\pm}_{\cquark\cquark}}}\xspace}
\def\Xiccp        {{\ensuremath{\Xires^{+}_{\cquark\cquark}}}\xspace}
\def\Xiccm        {{\ensuremath{\Xiresbar{}^{-}_{\cquark\cquark}}}\xspace}
\def\Xiccpm       {{\ensuremath{\XiOrXibar{}^{\pm}_{\cquark\cquark}}}\xspace}
\def\Omegaccp     {{\ensuremath{\Omegares^{+}_{\cquark\cquark}}}\xspace}
\def\Omegaccm     {{\ensuremath{\Omegaresbar{}^{-}_{\cquark\cquark}}}\xspace}
\def\Omegaccpm    {{\ensuremath{\OmegaOrOmegabar{}^{\pm}_{\cquark\cquark}}}\xspace}


%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays

%% Lifetimes

%% Masses

%% EW theory, groups

%% QCD parameters

%% CKM, CP violation

%% Oscillations

%% Tagging

%% Key decay channels

%% Rare decays

%% Wilson coefficients and operators

%% Charm

%% QM


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Energy and momentum
%%% Aliases that are in the appropriate mixed case.
\def\TeV   {\tev}
\def\GeV   {\gev}
\def\MeV   {\mev}
\def\keV   {\kev}
\def\eV    {\ev}
\def\GeVc  {\gevc}
\def\MeVc  {\mevc}
\def\GeVcc {\gevcc}
\def\MeVcc {\mevcc}

%%% Versions that do not have the leading and trailing spaces
\newcommand{\TeVnosp}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}}{\ensuremath{\mathrm{Te\kern -0.1em V}}}}
\newcommand{\GeVnosp}{\ensuremath{\mathrm{Ge\kern -0.1em V}}}
\newcommand{\MeVnosp}{\ensuremath{\mathrm{Me\kern -0.1em V}}}
\newcommand{\keVnosp}{\ensuremath{\mathrm{ke\kern -0.1em V}}}
\newcommand{\eVnosp}{\ensuremath{\mathrm{e\kern -0.1em V}}}
\newcommand{\GeVcnosp}{\ensuremath{{\mathrm{Ge\kern -0.1em V\!/}c}}}
\newcommand{\MeVcnosp}{\ensuremath{{\mathrm{Me\kern -0.1em V\!/}c}}}
\newcommand{\GeVccnosp}{\ensuremath{{\mathrm{Ge\kern -0.1em V\!/}c^2}}}
\newcommand{\MeVccnosp}{\ensuremath{{\mathrm{Me\kern -0.1em V\!/}c^2}}}
\newcommand{\GeVGeVccccnosp}{\ensuremath{{\mathrm{Ge\kern -0.1em V^2\!/}c^4}}}

%% Distance and area
%%% Alternate versions of areas
\def\msq        {\ensuremath{{\mathrm{ \,m}}^2}\xspace}
\def\cmsq       {\ensuremath{{\mathrm{ \,cm}}^2}\xspace}
\def\mmsq       {\ensuremath{{\mathrm{ \,mm}}^2}\xspace}
\def\mumsq      {\ensuremath{{\,\upmu\mathrm{m}^2}}\xspace}

%%% Versions that do not have the leading and trailing spaces
\def\kmnosp     {\ensuremath{\mathrm{km}}}
\def\mnosp      {\ensuremath{\mathrm{m}}}
\def\msqnosp    {\ensuremath{{\mathrm{m}}^2}}
\def\cmnosp     {\ensuremath{\mathrm{cm}}}
\def\cmsqnosp   {\ensuremath{{\mathrm{cm}}^2}}
\def\mmnosp     {\ensuremath{\mathrm{mm}}}
\def\mmsqnosp   {\ensuremath{{\mathrm{mm}}^2}}
\def\mumnosp    {\ensuremath{{\upmu\mathrm{m}}}}
\def\mumsqnosp  {\ensuremath{{\upmu\mathrm{m}^2}}}
\def\nmnosp     {\ensuremath{\mathrm{nm}}}
\def\fmnosp     {\ensuremath{\mathrm{fm}}}
\def\barnnosp   {\ensuremath{\mathrm{b}}}
\def\mbarnnosp  {\ensuremath{\mathrm{mb}}}
\def\mubnosp    {\ensuremath{{\mathrm{\upmu b}}}}
\def\nbnosp     {\ensuremath{\mathrm{nb}}}
\def\invnbnosp  {\ensuremath{\mbox{nb}^{-1}}}
\def\pbnosp     {\ensuremath{\mathrm{pb}}}
\def\invpbnosp  {\ensuremath{\mbox{pb}^{-1}}}
\def\fbnosp     {\ensuremath{\mbox{fb}}}
\def\invfbnosp  {\ensuremath{\mbox{fb}^{-1}}}
\def\abnosp     {\ensuremath{\mbox{ab}}}
\def\invabnosp  {\ensuremath{\mbox{ab}^{-1}}}

%% Time 
%%% Aliases that are in the appropriate mixed case.
\def\MHz  {\ensuremath{{\mathrm{ \,MHz}}}\xspace}
\def\kHz  {\ensuremath{{\mathrm{ \,kHz}}}\xspace}
\def\Hz   {\ensuremath{{\mathrm{ \,Hz}}}\xspace}

%%% Versions that do not have the leading and trailing spaces
\def\secnosp  {\ensuremath{\mathrm{{s}}}}
\def\msnosp   {\ensuremath{{\mathrm{ms}}}}
\def\musnosp  {\ensuremath{{\upmu{\mathrm{ s}}}}}
\def\nsnosp   {\ensuremath{{\mathrm{ns}}}}
\def\psnosp   {\ensuremath{{\mathrm{ps}}}}
\def\fsnosp   {\ensuremath{\mathrm{fs}}}

\def\MHznosp  {\ensuremath{{\mathrm{MHz}}}}
\def\kHznosp  {\ensuremath{{\mathrm{kHz}}}}
\def\Hznosp   {\ensuremath{{\mathrm{Hz}}}}

\def\invpsnosp {\ensuremath{{\mathrm{ps^{-1}}}}}
\def\invnsnosp {\ensuremath{{\mathrm{ns^{-1}}}}}

\def\yrnosp   {\ensuremath{\mathrm{yr}}}
\def\hrnosp   {\ensuremath{\mathrm{hr}}}

%% Temperature

%% Material lengths, radiation

%% Uncertainties

%% Math
%%% Some macros for derivatives.  Defaults are inline macros.
\newcommand{\dxdy}[2]{\ensuremath{\mathrm{d}\hspace{-0.1em}#1/\mathrm{d}#2}\xspace}
\newcommand{\altdxdy}[2]{\ensuremath{\frac{\mathrm{d}\hspace{-0.1em}#1}{\mathrm{d}\hspace{-0.1em}#2}}\xspace}
\newcommand{\ddxdydz}[3]{\ensuremath{\mathrm{d}^{2}\hspace{-0.1em}#1/\mathrm{d}\hspace{-0.1em}#2\mathrm{d}\hspace{-0.1em}#3}\xspace}
\newcommand{\altddxdydz}[3]{\ensuremath{\frac{\mathrm{d}^{2}\hspace{-0.1em}#1}{\mathrm{d}\hspace{-0.1em}#2\mathrm{d}\hspace{-0.1em}#3}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
%%% Alternate versions of transverse symbols
\def\pT         {\mbox{$p_{\mathrm{ T}}$}\xspace}
\def\ET         {\mbox{$E_{\mathrm{ T}}$}\xspace}

%% PID
%%% Alternative versions of PID symbols typeset with a base macro.
\newcommand{\DLL}[2]{\ensuremath{\mathrm{DLL}_{#1#2}}\xspace}
\def\dllkpi     {\DLL{\kaon}{\pion}}
\def\dllppi     {\DLL{\proton}{\pion}}
\def\dllepi     {\DLL{\electron}{\pion}}
\def\dllmupi    {\DLL{\muon}{\pion}}

%%% Alternative versions of PID symbols as logs of likelihood ratios.
\newcommand{\LLR}[2]{\ensuremath{\log\left(\mathcal{L}_{#1}/\mathcal{L}_{#2}\right)}\xspace}
\def\dllaltkpi     {\LLR{\kaon}{\pion}}
\def\dllaltppi     {\LLR{\proton}{\pion}}
\def\dllaltepi     {\LLR{\electron}{\pion}}
\def\dllaltmupi    {\LLR{\muon}{\pion}}


%% Geometry

%% Accelerator

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
\def\genxicc      {\mbox{\textsc{GENXICC}}\xspace}
\def\genxiccone   {\mbox{\textsc{GenXicc1.0}}\xspace}
\def\genxicctwo   {\mbox{\textsc{GenXicc2.0}}\xspace}

%% Languages

%% Data processing

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies

%% Detector components, electronics

%% Chemical symbols
\def\Xiccbare     {{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xibcbare     {{\ensuremath{\Xires_{\bquark\cquark}}}\xspace}
\def\Xibbbare     {{\ensuremath{\Xires_{\bquark\bquark}}}\xspace}


%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%


==> lhcb-symbols-def.tex <==
%%% $Id: lhcb-symbols-def.tex 125058 2018-12-06 11:25:21Z pkoppenb $
%%% ======================================================================
%%% Purpose: Standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes
%%% Maintainer : Ulrik Egede (2010 - 2012)
%%% Maintainer : Rolf Oldeman (2012 - 2014)
%%% Maintainer : Patrick Koppenburg (2018--2020)
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%
%%% For upper greek letters, Xires and Xiresbar will be the particles without the charge
%%% States with charge are called Xiz and Xim  
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\lhcb   {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\belletwo {\mbox{Belle~II}\xspace}
\def\besiii {\mbox{BESIII}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
%%%\def\argus  {\mbox{ARGUS}\xspace}
%%%\def\uaone  {\mbox{UA1}\xspace}
%%%\def\uatwo  {\mbox{UA2}\xspace}
%%%\def\ux85 {\mbox{UX85}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}
\def\bfactories {\mbox{\B Factories}\xspace}
\def\bfactory   {\mbox{\B Factory}\xspace}
\def\upgradeone {\mbox{Upgrade~I}\xspace}
\def\upgradetwo {\mbox{Upgrade~II}\xspace}

%% LHCb sub-detectors and sub-systems

%%%\def\pu     {PU\xspace}
\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
\def\herschel {\mbox{\textsc{HeRSCheL}}\xspace}
%%%\def\Tone   {T1\xspace}
%%%\def\Ttwo   {T2\xspace}
%%%\def\Tthree {T3\xspace}
%%%\def\Mone   {M1\xspace}
%%%\def\Mtwo   {M2\xspace}
%%%\def\Mthree {M3\xspace}
%%%\def\Mfour  {M4\xspace}
%%%\def\Mfive  {M5\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
%%%\def\bcm    {BCM\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\def\ode    {ODE\xspace}
\def\daq    {DAQ\xspace}
\def\tfc    {TFC\xspace}
\def\ecs    {ECS\xspace}
\def\lone   {L0\xspace}
\def\hlt    {HLT\xspace}
\def\hltone {HLT1\xspace}
\def\hlttwo {HLT2\xspace}

%%% Upright (not slanted) Particles

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi         {\ensuremath{\Xi}\xspace}                 
 \def\PLambda     {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon    {\ensuremath{\Upsilon}\xspace}                 

 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
 \def\thebaroffset{0.0em}
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}
 \def\thebaroffset{0.18em}
}
\newcommand{\offsetoverline}[2][\thebaroffset]{\kern #1\overline{\kern -#1 #2}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}


%% Leptons

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}   % electron negative (\em is taken)
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\emp        {{\ensuremath{\Pe^\mp}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}
%%%\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace} % muon negative (\mum is taken)
\def\mupm       {{\ensuremath{\Pmu^\pm}}\xspace} 
\def\mump       {{\ensuremath{\Pmu^\mp}}\xspace} 
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\taupm      {{\ensuremath{\Ptau^\pm}}\xspace}
\def\taump      {{\ensuremath{\Ptau^\mp}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
%%%\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
%%%\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
%%%\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
%%%\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}
%%%\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

%% Quarks

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

%% Light mesons

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
%%% do NOT use ensuremath here, and keep indent
\def\Kbar    {{\ensuremath{\offsetoverline{\PK}}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \PK}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\mathrm{S}}}}\xspace}
\def\Vzero   {{\ensuremath{V^0}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\mathrm{L}}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}
\def\KorKbarz {\ensuremath{\KorKbar^0}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

%% Charmed mesons

%%% do NOT use ensuremath here (and keep indent)
\def\Dbar    {{\ensuremath{\offsetoverline{\PD}}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \PD}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\theDstarz{{\ensuremath{\D^{*}(2007)^{0}}}\xspace}
\def\theDstarzb{{\ensuremath{\Dbar^{*}(2007)^{0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\theDstarp{{\ensuremath{\D^{*}(2010)^{+}}}\xspace}
\def\theDstarm{{\ensuremath{\D^{*}(2010)^{-}}}\xspace}
\def\theDstarpm{{\ensuremath{\D^{*}(2010)^{\pm}}}\xspace}
\def\theDstarmp{{\ensuremath{\D^{*}(2010)^{\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}

%% Beauty mesons
\def\B       {{\ensuremath{\PB}}\xspace}
\def\Bbar    {{\ensuremath{\offsetoverline{\PB}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \PB}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\BdorBdbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \Bd}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\BsorBsbar {\kern \thebaroffset\optbar{\kern -\thebaroffset \Bs}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}
\def\Bds     {{\ensuremath{\B_{(\squark)}^0}}\xspace}
\def\Bdsb    {{\ensuremath{\Bbar{}_{(\squark)}^0}}\xspace}
\def\BdorBs  {{\ensuremath{\Bbar{}_{(\squark)}^0}}\xspace}

%% Onia

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\chic     {{\ensuremath{\Pchi_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
\def\chicJ    {{\ensuremath{\Pchi_{\cquark J}}}\xspace}
\def\Upsilonres  {{\ensuremath{\PUpsilon}}\xspace}
\def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}
\def\OneS  {{\Y1S}}
\def\TwoS  {{\Y2S}}
\def\ThreeS{{\Y3S}}
\def\FourS {{\Y4S}}
\def\FiveS {{\Y5S}}
\def\chib     {{\ensuremath{\Pchi_{c}}}\xspace}
\def\chibzero {{\ensuremath{\Pchi_{\bquark 0}}}\xspace}
\def\chibone  {{\ensuremath{\Pchi_{\bquark 1}}}\xspace}
\def\chibtwo  {{\ensuremath{\Pchi_{\bquark 2}}}\xspace}
\def\chibJ    {{\ensuremath{\Pchi_{\bquark J}}}\xspace}

%% Light Baryons

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
%%% uds singlet
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\offsetoverline{\PLambda}}}\xspace}
\def\LorLbar     {\kern \thebaroffset\optbar{\kern -\thebaroffset \PLambda}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
%%% uus, uds, dds
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaz      {{\ensuremath{\Sigmares{}^0}}\xspace}
\def\Sigmap      {{\ensuremath{\Sigmares{}^+}}\xspace}
\def\Sigmam      {{\ensuremath{\Sigmares{}^-}}\xspace}
\def\Sigmaresbar {{\ensuremath{\offsetoverline{\Sigmares}}}\xspace}
\def\Sigmabarz   {{\ensuremath{\Sigmaresbar{}^0}}\xspace}
\def\Sigmabarp   {{\ensuremath{\Sigmaresbar{}^+}}\xspace}
\def\Sigmabarm   {{\ensuremath{\Sigmaresbar{}^-}}\xspace}
%%%  uss, dss
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiresz      {{\ensuremath{\Xires^0}}\xspace}
\def\Xiresm      {{\ensuremath{\Xires^-}}\xspace}
\def\Xiresbar    {{\ensuremath{\offsetoverline{\Xires}}}\xspace}
\def\Xiresbarz   {{\ensuremath{\Xiresbar^0}}\xspace}
\def\Xiresbarp   {{\ensuremath{\Xiresbar^+}}\xspace}
%%%  sss
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\offsetoverline{\POmega}}}\xspace}
\def\Omegam      {{\ensuremath{\Omegares^-}}\xspace}
\def\Omegabarp   {{\ensuremath{\Omegaresbar^+}}\xspace}

%% Charmed Baryons
\def\Lc          {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar       {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Xic         {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz        {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp        {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar      {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz     {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm     {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac      {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar   {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Xicc        {{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xiccbar     {{\ensuremath{\Xiresbar{}_{\cquark\cquark}}}\xspace}
\def\Xiccp       {{\ensuremath{\Xires^+_{\cquark\cquark}}}\xspace}
\def\Xiccpp      {{\ensuremath{\Xires^{++}_{\cquark\cquark}}}\xspace}
\def\Xiccbarm    {{\ensuremath{\Xiresbar{}_{\cquark\cquark}^-}}\xspace}
\def\Xiccbarmm   {{\ensuremath{\Xiresbar{}_{\cquark\cquark}^{--}}}\xspace}
\def\Omegacc     {{\ensuremath{\Omegares^+_{\cquark\cquark}}}\xspace}
\def\Omegaccbar  {{\ensuremath{\Omegaresbar{}_{\cquark\cquark}^-}}\xspace}
\def\Omegaccc    {{\ensuremath{\Omegares^{++}_{\cquark\cquark\cquark}}}\xspace}
\def\Omegacccbar {{\ensuremath{\Omegaresbar{}_{\cquark\cquark\cquark}^{--}}}\xspace}
\def\Omegaca      {{\ensuremath{\Omegares_{\cquark}(3000)^{0}}}\xspace}
\def\Omegacb      {{\ensuremath{\Omegares_{\cquark}(3050)^{0}}}\xspace}
\def\Omegacd      {{\ensuremath{\Omegares_{\cquark}(3066)^{0}}}\xspace}
\def\Omegace      {{\ensuremath{\Omegares_{\cquark}(3090)^{0}}}\xspace}
\def\Omegacf      {{\ensuremath{\Omegares_{\cquark}(3119)^{0}}}\xspace}
%% Beauty Baryons

\def\Lb           {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar        {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Sigmab       {{\ensuremath{\Sigmares_\bquark}}\xspace}
\def\Sigmabp      {{\ensuremath{\Sigmares_\bquark^+}}\xspace}
\def\Sigmabz      {{\ensuremath{\Sigmares_\bquark^0}}\xspace}
\def\Sigmabm      {{\ensuremath{\Sigmares_\bquark^-}}\xspace}
\def\Sigmabpm     {{\ensuremath{\Sigmares_\bquark^\pm}}\xspace}
\def\Sigmabbar    {{\ensuremath{\Sigmaresbar_\bquark}}\xspace}
\def\Sigmabbarp   {{\ensuremath{\Sigmaresbar_\bquark^+}}\xspace}
\def\Sigmabbarz   {{\ensuremath{\Sigmaresbar_\bquark^0}}\xspace}
\def\Sigmabbarm   {{\ensuremath{\Sigmaresbar_\bquark^-}}\xspace}
\def\Sigmabbarpm  {{\ensuremath{\Sigmaresbar_\bquark^-}}\xspace}
\def\Xib          {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz         {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm         {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar       {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz      {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp      {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Omegab       {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar    {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\mathcal{B}}}\xspace}
\def\BR         {\BF}
\def\BRvis      {{\ensuremath{\BR_{\mathrm{{vis}}}}}}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace} 
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% Lifetimes
\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\mathrm{ L}}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\mathrm{ H}}}}\xspace}

%% Masses
\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

%% EW theory, groups
\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

%% QCD parameters
\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

%% CKM, \boldmath \CP violation

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}
\def\T                 {{\ensuremath{T}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

%% Oscillations

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\mathrm{ L}}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\mathrm{ H}}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\mathcal{A}}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\mathcal{A}}^{\mathrm{ dir}}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\mathcal{A}}^{\mathrm{ mix}}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\mathcal{A}}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\mathrm{ det}}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\mathrm{ rec/det}}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\mathrm{ sel/rec}}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\mathrm{ trg/sel}}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\mathrm{ tot}}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\mathrm{comb}}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\mathrm{tag}}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\mathrm{tag}}^{\mathrm{comb}}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\mathrm{eff}}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\mathrm{eff}}^{\mathrm{comb}}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{Pr}}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{LL}}}}\xspace}

%% Key decay channels

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}
\def\Cpipi        {\ensuremath{C_{\pip\pim}}\xspace}
\def\Spipi        {\ensuremath{S_{\pip\pim}}\xspace}
\def\CKK          {\ensuremath{C_{\Kp\Km}}\xspace}
\def\SKK          {\ensuremath{S_{\Kp\Km}}\xspace}
\def\ADGKK        {\ensuremath{A^{\DG}_{\Kp\Km}}\xspace}

%% Rare decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\Bsee     {\decay{\Bs}{\epem}}
\def\Bdee     {\decay{\Bd}{\epem}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}                    % 7

%% Charm

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
%%%\def\kpi        {\ensuremath{\PK\Ppi}\xspace}
%%%\def\kk         {\ensuremath{\PK\PK}\xspace}
%%%\def\dkpi       {\decay{\PD}{\PK\Ppi}}
%%%\def\dkk        {\decay{\PD}{\PK\PK}}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units (these macros add a small space in front)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\nospaceunit}[1]{\ensuremath{\text{#1}}}       
\newcommand{\aunit}[1]{\ensuremath{\text{\,#1}}}       
\newcommand{\unit}[1]{\aunit{#1}\xspace}                   % {kg}   

%% Energy and momentum 
\newcommand{\tev}{\aunit{Te\kern -0.1em V}\xspace}
\newcommand{\gev}{\aunit{Ge\kern -0.1em V}\xspace}
\newcommand{\mev}{\aunit{Me\kern -0.1em V}\xspace}
\newcommand{\kev}{\aunit{ke\kern -0.1em V}\xspace}
\newcommand{\ev}{\aunit{e\kern -0.1em V}\xspace}
\newcommand{\mevc}{\ensuremath{\aunit{Me\kern -0.1em V\!/}c}\xspace}
\newcommand{\gevc}{\ensuremath{\aunit{Ge\kern -0.1em V\!/}c}\xspace}
\newcommand{\mevcc}{\ensuremath{\aunit{Me\kern -0.1em V\!/}c^2}\xspace}
\newcommand{\gevcc}{\ensuremath{\aunit{Ge\kern -0.1em V\!/}c^2}\xspace}
\newcommand{\gevgevcc}{\ensuremath{\gev^2\!/c^2}\xspace} % for \pt^2 in CEP
\newcommand{\gevgevcccc}{\ensuremath{\gev^2\!/c^4}\xspace} % for q^2

%% Distance and area (these macros add a small space)
\def\km   {\aunit{km}\xspace}
\def\m    {\aunit{m}\xspace}
\def\ma   {\ensuremath{\aunit{m}^2}\xspace}
\def\cm   {\aunit{cm}\xspace}
\def\cma  {\ensuremath{\aunit{cm}^2}\xspace}
\def\mm   {\aunit{mm}\xspace}
\def\mma  {\ensuremath{\aunit{mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\nospaceunit{m}}\xspace}
\def\muma {\ensuremath{\,\upmu\nospaceunit{m}^2}\xspace}
\def\nm   {\aunit{nm}\xspace}
\def\fm   {\aunit{fm}\xspace}
\def\barn{\aunit{b}\xspace}
%%%\def\barnhyph{\ensuremath{\mathrm{ -b}}
\def\mbarn{\aunit{mb}\xspace}
\def\mub{\ensuremath{\,\upmu\nospaceunit{b}}\xspace}
%%%\def\mbarnhyph{\ensuremath{\mathrm{ -mb}}
\def\nb {\aunit{nb}\xspace}
\def\invnb {\ensuremath{\nb^{-1}}\xspace}
\def\pb {\aunit{pb}\xspace}
\def\invpb {\ensuremath{\pb^{-1}}\xspace}
\def\fb   {\ensuremath{\aunit{fb}}\xspace}
\def\invfb   {\ensuremath{\fb^{-1}}\xspace}
\def\ab   {\ensuremath{\aunit{ab}}\xspace}
\def\invab   {\ensuremath{\ab^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\aunit{s}}\xspace}
\def\ms   {\ensuremath{\aunit{ms}}\xspace}
\def\mus  {\ensuremath{\,\upmu\nospaceunit{s}}\xspace}
\def\ns   {\ensuremath{\aunit{ns}}\xspace}
\def\ps   {\ensuremath{\aunit{ps}}\xspace}
\def\fs   {\ensuremath{\aunit{fs}}\xspace}

\def\mhz  {\ensuremath{\aunit{MHz}}\xspace}
\def\khz  {\ensuremath{\aunit{kHz}}\xspace}
\def\hz   {\ensuremath{\aunit{Hz}}\xspace}

\def\invps{\ensuremath{\ps^{-1}}\xspace}
\def\invns{\ensuremath{\ns^{-1}}\xspace}

\def\yr   {\aunit{yr}\xspace}
\def\hr   {\aunit{hr}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{\text{C}}\xspace}
\def\degk {\aunit{K}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{\rm int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{n_\nospaceunit{eq}}\xspace}
\def\neqcmcm {\ensuremath{\neutroneq/\nospaceunit{cm}^2}\xspace}
\def\kRad {\aunit{kRad}\xspace}
\def\MRad {\aunit{MRad}\xspace}
\def\ci {\aunit{Ci}\xspace}
\def\mci {\aunit{mCi}\xspace}

%% Uncertainties
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\aunit{(stat)}\xspace}
\newcommand{\syst}{\aunit{(syst)}\xspace}

%% Maths

\def\order{{\ensuremath{\mathcal{O}}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\text{IP}}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\text{VS}}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\text{vtx}}}\xspace}
\newcommand{\chisqvtxndf}{\ensuremath{\chi^2_{\text{vtx}}/\mathrm{ndf}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}
\def\sFit{\mbox{\em sFit}\xspace}
%%%\def\sWeight{\mbox{\em sWeight}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}
\def\sqsnn {\ensuremath{\protect\sqrt{s_{\scriptscriptstyle\text{NN}}}}\xspace}
\def\pt         {\ensuremath{p_{\mathrm{T}}}\xspace}
\def\ptsq       {\ensuremath{p_{\mathrm{T}}^2}\xspace}
\def\ptot       {\ensuremath{p}\xspace}
\def\et         {\ensuremath{E_{\mathrm{T}}}\xspace}
\def\mt         {\ensuremath{M_{\mathrm{T}}}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
%% PID
\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}
%% Geometry
%%%\def\mphi       {\mbox{$\phi$}\xspace}
%%%\def\mtheta     {\mbox{$\theta$}\xspace}
%%%\def\ctheta     {\mbox{$\cos\theta$}\xspace}
%%%\def\stheta     {\mbox{$\sin\theta$}\xspace}
%%%\def\ttheta     {\mbox{$\tan\theta$}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\murad{\ensuremath{\,\upmu\nospaceunit{rad}}\xspace}
\def\mrad{\aunit{mrad}}
\def\rad{\aunit{rad}}

%% Accelerator
\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}  % {2 \,\invfb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
%%%\def\ansys      {\mbox{\textsc{Ansys}}\xspace}
\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
%%%\def\erasmus    {\mbox{\textsc{Erasmus}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
%%%\def\garfield   {\mbox{\textsc{Garfield}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
%%%\def\pyroot     {\mbox{\textsc{PyRoot}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
%%%\def\tosca      {\mbox{\textsc{Tosca}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
%%%\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{svn}}\xspace}
\def\git        {\mbox{\textsc{git}}\xspace}
\def\latex      {\mbox{\LaTeX}\xspace}

%% Data processing
\def\kbit          {\aunit{kbit}\xspace}
\def\kbps        {\aunit{kbit/s}\xspace}
\def\kbytes     {\aunit{kB}\xspace}
\def\kbyps      {\aunit{kB/s}\xspace}
\def\mbit          {\aunit{Mbit}\xspace}
\def\mbps        {\aunit{Mbit/s}\xspace}
\def\mbytes     {\aunit{MB}\xspace}
\def\mbyps      {\aunit{MB/s}\xspace}
\def\gbit          {\aunit{Gbit}\xspace}
\def\gbps        {\aunit{Gbit/s}\xspace}
\def\gbytes     {\aunit{GB}\xspace}
\def\gbyps      {\aunit{GB/s}\xspace}
\def\tbit          {\aunit{Tbit}\xspace}
\def\tbps        {\aunit{Tbit/s}\xspace}
\def\tbytes     {\aunit{TB}\xspace}
\def\tbyps      {\aunit{TB/s}\xspace}
\def\dst        {DST\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies
\def\nonn {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\ponn {\ensuremath{\mathrm{{ \mathit{p^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\nonp {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{p}}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

%% Detector components, electronics
\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

%% Chemical symbols
\def\cfourften     {\ensuremath{\mathrm{ C_4 F_{10}}}\xspace}
\def\cffour        {\ensuremath{\mathrm{ CF_4}}\xspace}
\def\cotwo         {\ensuremath{\mathrm{ CO_2}}\xspace} 
\def\csixffouteen  {\ensuremath{\mathrm{ C_6 F_{14}}}\xspace} 
\def\mgftwo     {\ensuremath{\mathrm{ Mg F_2}}\xspace} 
\def\siotwo     {\ensuremath{\mathrm{ SiO_2}}\xspace} 

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}


==> preamble.tex <==
% THis file contains all the default packages and modifications for
% LHCb formatting

%% %%%%%%%%%%%%%%%%%%
%%  Page formatting
%% %%%%%%%%%%%%%%%%%%
%%\usepackage[margin=1in]{geometry}
\usepackage[top=1in, bottom=1.25in, left=1in, right=1in]{geometry}

% fallback for manual settings... uncomment if the geometry package is not available
%
%\voffset=-11mm
%\textheight=220mm
%\textwidth=160mm
%\oddsidemargin=0mm
%\evensidemargin=0mm

\columnsep=5mm
\addtolength{\belowcaptionskip}{0.5em}

\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.8} % changed from 0.99
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}

% Allow the page size to vary a bit ...
\raggedbottom
% To avoid Latex to be too fussy with line breaking ...
\sloppy

%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%% 
\usepackage{microtype}
\usepackage{lineno}  % for line numbering during review
\usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbold
\usepackage{caption} %these three command get the figure and table captions automatically small
\renewcommand{\captionfont}{\small}
\renewcommand{\captionlabelfont}{\small}

%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
\usepackage{color}
\usepackage{colortbl}
\graphicspath{{./figs/}} % Make Latex search fig subdir for figures
\DeclareGraphicsExtensions{.pdf,.PDF,png,.PNG}

%% Math
\usepackage{amsmath} % Adds a large collection of math symbols
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/viewtopic.php?f=5&t=163
%%
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
\expandafter\let\csname oldend#1\expandafter\endcsname\csname
end#1\endcsname
 \renewenvironment{#1}%
   {\linenomath\csname old#1\endcsname}%
   {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
\patchBothAmsMathEnvironmentsForLineno{eqnarray}%
}

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.

\usepackage{hyperxmp}

\usepackage[pdftex,
            pdfauthor={\paperauthors},
            pdftitle={\paperasciititle},
            pdfkeywords={\paperkeywords},
            pdfcopyright={Copyright (C) \papercopyright},
            pdflicenseurl={\paperlicenceurl}]{hyperref}

% overleaf comments
\usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}

\usepackage[all]{hypcap} % Internal hyperlinks to floats.

\input{lhcb-symbols-def} % Add in the predefined LHCb symbols

% Additional symbols that are not in lhcb-symbols-def
\input{fixed-symbols-def} 
\input{user-symbols-def}

% for number display
\usepackage{siunitx}
\sisetup{separate-uncertainty}

% Make this the last packages you include before the \begin{document}
\usepackage{cite} % Allows for ranges in citations
\usepackage{mciteplus}


==> title-LHCb-PAPER.tex <==
% $Id: title-LHCb-PAPER.tex 122889 2018-08-17 17:59:55Z pkoppenb $
% ===============================================================================
% Purpose: LHCb-PAPER journal paper title page template
% Author: 
% Created on: 2010-09-25
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}
\pagenumbering{roman}

% Header ---------------------------------------------------
\vspace*{-1.5cm}
\centerline{\large EUROPEAN ORGANIZATION FOR NUCLEAR RESEARCH (CERN)}
\vspace*{1.5cm}
\noindent
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r@{\extracolsep{0pt}}}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-1.5cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{Figs/lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{Figs/lhcb-logo.eps}} & &}%
\\
 & & CERN-EP-2021-068 \\  % ID 
 & & LHCb-PAPER-2021-011 \\  % ID 
 & & \today \\ % Date - Can also hardwire e.g.: 23 March 2010
 & & \\
% not in paper \hline
\end{tabular*}

\vspace*{4.0cm}

% Title --------------------------------------------------
{\normalfont\bfseries\boldmath\huge
\begin{center}
% DO NOT EDIT HERE. Instead edit macro in main.tex to keep metadata correct
  \papertitle 
\end{center}
}

\vspace*{2.0cm}

% Authors -------------------------------------------------
\begin{center}
%In the footnote, replace 'paper' by 'Letter' in case of submission to PRL or PLB 
% Edit macro in main.tex to keep metadata correct
\paperauthors\footnote{Authors are listed at the end of this paper.}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
  A search for the doubly charmed baryon \Omegacc with the decay mode $\Omegacc\to\Xicp\Km\pip$ is performed 
  using proton-proton collision data at a centre-of-mass energy of
  13\tev collected by the \lhcb experiment from 2016 to 2018,
  corresponding to an integrated luminosity of 5.4\invfb. No significant signal is observed within the invariant mass range of 3.6 to 4.0\gevcc. Upper limits are set on the ratio $R$ of the production cross-section times the total branching fraction of the $\Omegacc\to\Xicp\Km\pip$ decay with respect to the $\Xiccpp\to\Lc\Km\pip\pip$ decay. Upper limits at 95\% credibility level for $R$ in the range  $0.005$ to $0.11$ are obtained for different hypotheses on the \Omegacc mass and lifetime in the rapidity range from 2.0 to 4.5 and transverse momentum range from 4 to 15\gevc.
  
\end{abstract}

\vspace*{2.0cm}

\begin{center}
  Submitted to
  Science China Physics, Mechanics \& Astronomy
\end{center}

\vspace{\fill}

{\footnotesize 
% Edit macro in main.tex to keep metadata correct
\centerline{\copyright~\papercopyright. \href{\paperlicenceurl}{\paperlicence}.}}
\vspace*{2mm}

\end{titlepage}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}
%\newpage
%
%% Author List ----------------------------
%%  You need to get a new author list!
%\input{LHCb_authorlist.tex}
%
%The author list for journal publications is provided by the Membership Committee shortly after 'approval to go to paper' has been given.
%%It will be made available on the page
%%\verb!http://www.physik.uzh.ch/~strauman/forMemCo/LHCb-PAPER-XXXX-XXX/! .
%It will be sent to you by email shortly after a paper number has beens assigned.
%The author list should be included already at first circulation, 
%to allow new members of the collaboration to verify whether they have been included correctly.
%Occasionally a misspelled name is corrected or associated institutions become full members.
%In that case, a new author list will be sent to you.
%In case line numbering doesn't work well after including the authorlist, try moving the \verb!\bigskip! after the last author to a separate line.
%
%
%The authorship for Conference Reports should be ``The LHCb
%  collaboration'', with a footnote giving the name(s) of the contact
%  author(s), but without the full list of collaboration names.



\cleardoublepage









==> typography.tex <==
\section{Typography}
\label{sec:typography}

The use of the \latex typesetting symbols defined in the file
\texttt{lhcb-symbols-def.tex} and detailed in the appendices of this
document is strongly encouraged as it will make it much easier to
follow the recommendation set out below.

\begin{enumerate}

\item \lhcb is typeset with a normal (roman) lowercase b.

\item Titles are in bold face, and usually only the first word is
  capitalised.

\item Mathematical symbols and particle names should also be typeset
  in bold when appearing in titles.

\item Units are in roman type, except for constants such as $c$ or $h$
  that are italic: \gev, \gevcc.  The unit should be separated from
  the value with a thin space (``\verb!\,!''),
  and they should not be broken over two lines.
  Correct spacing is automatic when using predefined units inside math mode: \verb!$3.0\gev$! $\to 3.0\gev$.
  Spacing goes wrong when using predefined units outside math mode AND forcing extra space:
  \verb!3.0\,\gev! $\to$ 3.0\,\gev or worse:   \verb!3.0~\gev! $\to$ 3.0~\gev. 

\item  If factors of $c$ are kept, they should be used both for masses and
  momenta, \eg $p=5.2\gevc$ (or $\gev c^{-1}$), $m = 3.1\gevcc$ (or $\gev c^{-2}$). If they are dropped this
  should be done consistently throughout, and a note should be added
  at the first instance to indicate that units are taken with $c=1$.
  Note that there is no consensus on whether decay widths $\Gamma$ are
  in \mev or \mevcc (the former is more common).
  Both are accepted if consistent. 

\item The \% sign should not be separated from the number that precedes it: 5\%, not 5 \%. 
A thin space is also acceptable: 5\,\%, but should be applied consistently throughout the paper.

\item Ranges should be formatted consistently. The recommended form is to use a dash with no spacing around it: 
7--8\gev, obtained as \verb!7--8\gev!. Another possibility is ``7 to 8\gev''.

\item Italic is preferred for particle names (although roman is
  acceptable, if applied consistently throughout).  Particle Data
  Group conventions should generally be followed: \Bd (no need for a
  ``d'' subscript), \decay{\Bs}{\jpsi\phi}, \Bsb,
  (note the long bar, obtained with \verb!\overline!, in contrast to the discouraged short \verb!\bar{B}! resulting in $\bar{B}$), \KS (note the
  uppercase roman type ``S''). 
  This is most easily achieved by using the predefined symbols described in 
  Appendix~\ref{sec:listofsymbols}.

  Italic is also used for particles whose name is an uppercase Greek letter:
  \Upsilonres, \Deltares, \Xires, \Lambdares, \Sigmares, \Omegares, typeset as
  \verb!\Upsilonres!, \verb!\Deltares!, \verb!\Xires!, \verb!\Lambdares!, \verb!\Sigmares!, \verb!\Omegares! (or with the appropriate macros adding charge and subscripts). Paper titles in the bibliography must be adapted accordingly.
  Note that the \Lz baryon has no zero, while the \Lb baryon has one. That's historical.
  
\item Unless there is a good reason not to, the charge of a particle should be
  specified if there is any possible ambiguity 
  ($m(\Kp\Km)$ instead of $m(KK)$, which could refer to neutral kaons).


\item Decay chains can be written in several ways, depending on the complexity and the number of times it occurs. Unless there is a good reason not to, usage of a particular type should be consistent within the paper.
Examples are: 
\decay{\Dsp}{\phi\pip}, with \decay{\phi}{\Kp\Km}; 
\decay{\Dsp}{\phi\pip} (\decay{\phi}{\Kp\Km});  
\decay{\Dsp}{\phi(}{\Kp\Km)\pip}; or
\decay{\Dsp}{[\Kp\Km]_\phi\pip}.

\item Variables are usually italic: $V$ is a voltage (variable), while
  1 V is a volt (unit). Also in combined expressions: $Q$-value, $z$-scale, $R$-parity \etc

\item Subscripts and superscripts are roman type when they refer to a word (such as T
  for transverse) and italic when they refer to a variable (such as
  $t$ for time): \pt, \dms, $t_{\mathrm{rec}}$.

%  This is a test: $f_{\pt}$.

\item Standard function names are in roman type: \eg $\cos$, $\sin$
  and $\exp$.

\item Figure, Section, Equation, Chapter and Reference should be
  abbreviated as Fig., Sect. (or alternatively Sec.), Eq., Chap.\ and
  Ref.\ respectively, when they refer to a particular (numbered) item,
  except when they start a sentence. Table and Appendix are not
  abbreviated.  The plural form of abbreviation keeps the point after
  the s, \eg Figs.~1 and~2. Equations may be referred to either with 
  (``Eq.~(1)'') or without (``Eq.~1'') parentheses, 
  but it should be consistent within the paper.

\item Common abbreviations derived from Latin such as ``for example''
  (\eg), ``in other words'' (\ie), ``and so forth'' (\etc), ``and
  others'' (\etal), ``versus'' (\vs) can be used, with the typography
  shown, but not excessively; other more esoteric abbreviations should be avoided.
  

\item Units, material and particle names are usually lower case if
  spelled out, but often capitalised if abbreviated: amps (A), gauss
  (G), lead (Pb), silicon (Si), kaon (\kaon), but proton (\proton).

%\item The prefix for 1000 (k, \eg kV) should not be confused with
%  that used in computing (K, which strictly speaking denotes $2^{10}$,
%  \eg KB).

\item Counting numbers are usually written in words if they start a
  sentence or if they have a value of ten or below in descriptive
  text (\ie not including figure numbers such as ``Fig.\ 4'', or
  values followed by a unit such as ``4\,cm'').
  The word 'unity' can be useful to express the special meaning of
  the number one in expressions such as: 
``The BDT output takes values between zero and unity''.
% Numbers should not be
%  written as words if they by nature are real numbers that happen to
%  take an integer value, such as $\chisq/\mathrm{ndf} < 4$.

\item Numbers larger than 9999 have a small space between
  the multiples of thousand: \eg 10\,000 or 12\,345\,678.  The decimal
  point is indicated with a point rather than a comma: \eg 3.141.

\item We apply the rounding rules of the
  PDG~\cite{PDG2018}. The basic rule states that if the three
  highest order digits of the uncertainty lie between 100 and 354, we round
  to two significant digits. If they lie between 355 and 949, we round
  to one significant digit. Finally, if they lie between 950 and 999,
  we round up and keep two significant digits. In all cases,
  the central value is given with a precision that matches that of the
  uncertainty. So, for example, the result $0.827 \pm 0.119$ should be
  written as $0.83\pm 0.12$, $0.827\pm 0.367$ should turn into
  $0.8\pm 0.4$, and $14.674\pm0.964$ becomes $14.7\pm1.0$.
  When writing numbers with uncertainty components from
  different sources, \ie statistical and systematic uncertainties, the rule
  applies to the uncertainty with the best precision, so $0.827\pm
  0.367\stat\pm 0.179\syst$ goes to $0.83\pm 0.37\stat\pm 0.18\syst$ and
  $8.943\pm 0.123\stat\pm 0.995\syst$ goes to $8.94\pm 0.12\stat\pm
  1.00\syst$.

\item When rounding numbers, it should be avoided to pad with zeroes
  at the end. So $51237 \pm 4561$ should be rounded as $(5.12 \pm 0.46)
  \times 10^4$ rather than $51200 \pm 4600$. Zeroes are accepted for yields.

\item When rounding numbers in a table, some variation of the rounding
  rules above may be required to achieve uniformity.

\item Hyphenation should be used where necessary to avoid ambiguity,
  but not excessively. For example: ``big-toothed fish'' (to indicate
  that big refers to the teeth, not to the fish), but ``big white
  fish''.  A compound modifier often requires hyphenation
  (\CP-violating observables, \bquark-hadron decays, final-state
  radiation, second-order polynomial), even if the same combination in
  an adjective-noun combination does not (direct \CP violation, heavy
  \bquark hadrons, charmless final state).  Adverb-adjective
  combinations are not hyphenated if the adverb ends with 'ly':
  oppositely charged pions, kinematically similar decay.  Words
  beginning with ``all-'', ``cross-'', ``ex-'' and ``self-'' are
  hyphenated \eg\ cross-section and cross-check. ``two-dimensional''
  is hyphenated. Words beginning with small prefixes (like ``anti'',
  ``bi'', ``co'', ``contra'', ``counter'', ``de'', ``extra'', ``infra'',
  ``inter'', ``intra'', ``micro'', ``mid'', ``mis'', ``multi'', ``non'', ``over'',
  ``peri'', ``post'', ``pre'', ``pro'', ``proto'', ``pseudo'', ``re'', ``semi'',
  ``sub'', ``super'', ``supra'', ``trans'', ``tri'', ``ultra'', ``un'', ``under'' and
  ``whole'') are single words and should not be hyphenated
  \eg\ semileptonic, pseudorapidity, pseudoexperiment, multivariate,
  multidimensional, reweighted,\footnote{Note that we write weighted unless it's the second weighting} preselection, nonresonant, nonzero,
  nonparametric, nonrelativistic, antiparticle,
  misreconstructed and misidentified.

\item Minus signs should be in a proper font ($-1$), not just hyphens
  (-1); this applies to figure labels as well as the body of the text.
  In \latex, use math mode (between \verb!$$!'s) or make a dash (``\verb!--!'').
  In ROOT, use \verb!#minus! to get a normal-sized minus sign. 

\item Inverted commas (around a title, for example) should be a
  matching set of left- and right-handed pairs: ``Title''. The use of
  these should be avoided where possible.

\item Single symbols are preferred for variables in equations, \eg\
  \BF\ rather than BF for a branching fraction.

\item Parentheses are not usually required around a value and its
  uncertainty, before the unit, unless there is possible ambiguity: so
  \mbox{$\dms = 20 \pm 2\invps$} does not need parentheses,
  whereas \mbox{$f_d = (40 \pm 4)$\%} or \mbox{$x=(1.7\pm0.3)\times 10^{-6}$} does.
  The unit does not need to be repeated in
  expressions like \mbox{$1.2 < E < 2.4\gev$}.

\item The same number of decimal places should be given for all values
  in any one expression (\eg \mbox{$5.20 < m_B < 5.34\gevcc$}).

\item Apostrophes are best avoided for abbreviations: if the abbreviated term
  is capitalised or otherwise easily identified then the plural can simply add
  an s, otherwise it is best to rephrase: \eg HPDs, pions, rather
  than HPD's, \piz's, $\pion$s.

\item Particle labels, decay descriptors and mathematical functions are not nouns, and need often to be followed by a noun. 
Thus ``background from \decay{\Bd}{\pip\pim} decays'' instead of ``background from \decay{\Bd}{\pip\pim}'',
and ``the width of the Gaussian function'' instead of ``the width of the Gaussian''.

\item In equations with multidimensional integrations or differentiations, the differential terms should be separated by a thin space and the $\rm d$ should be in roman.
Thus $\int f(x,y) {\rm d}x\,{\rm d}y$ instead $\int f(x,y) {\rm d}x{\rm d}y$ and
$\frac{{\rm d}^2\Gamma}{{\rm d}x\,{\rm d}Q^2}$ instead of $\frac{{\rm d}^2\Gamma}{{\rm d}x{\rm d}Q^2}$.
% The d's are allowed in either roman or italic font, but should be consistent throughout the paper.

\item Double-barrelled names are typeset with a hyphen (\verb!-!), as in Gell-Mann, but joined named use an n-dash (\verb!--!), as in Breit--Wigner. 

\item Avoid gendered words. Mother is rarely needed. Daughter can be a decay product or a final-state particle. Bachelor can be replaced by companion.
\end{enumerate}


==> user-symbols-def.tex <==
% Additional symbols to make things more consistent and convinient

% Xiccpp2LcKPiPi result
\def\Xiccmass          {{\ensuremath{3621.40 \pm 0.72 \stat \pm 0.31 \syst \mevcc}}\xspace}
\def\XiccmassOneDigit  {{\ensuremath{3621.4 \pm 0.7 \stat \pm 0.3 \syst \mevcc}}\xspace}
\def\XiccDeltaMass {{\ensuremath{1334.94 \pm 0.72 \stat \pm 0.27 \syst \mevcc}}\xspace}

\renewcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bracket}[3]{\ensuremath{\langle #1|#2|#3\rangle}} % <a|B|c>
\def\max   {\ensuremath{{\rm max}}\xspace} %max
\def\min   {\ensuremath{{\rm min}}\xspace} %min
\def\Tr   {\ensuremath{{\rm Tr}}\xspace} %trace
\def\px   {\ensuremath{p_x}\xspace} %px
\def\py   {\ensuremath{p_y}\xspace} %py
\def\pz   {\ensuremath{p_z}\xspace} %pz

% Particle name
\def\Xicc{{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xiccp{{\ensuremath{\Xires_{\cquark\cquark}^{+}}}\xspace}
\def\Xiccpp{{\ensuremath{\Xires_{\cquark\cquark}^{++}}}\xspace}
\def\Omegaccbare{{\ensuremath{\Omegares_{\cquark\cquark}}}\xspace}
\def\Omegacc{{\ensuremath{\Omegares^{+}_{\cquark\cquark}}}\xspace}
\def\XiccppDecay{{\ensuremath{\Xiccpp\to\Lc\Km\pip\pip}}\xspace}
\def\XiccpDecay{{\ensuremath{\Xiccp\to\Lc\Km\pip}}\xspace}
\def\LcDecay{{\ensuremath{\Lc\to p\Km\pip}}\xspace}
\def\finalstate{{\ensuremath{\Lc\Km\pip}}\xspace}

% log IPCHI2
\def\logchisqip{{\ensuremath{\log_{10}(\chisqip)}}\xspace}

%Mass difference corrected by Lc mass
\def\DM{\ensuremath{\rm DM}\xspace}
%Units
\def\mb {\ensuremath{\rm \,mb}\xspace}
% for force
\def\UNewton   {\ensuremath{\rm \,N}\xspace} %Newton
% for mass
\def\kg   {\ensuremath{\rm \,kg}\xspace} %kg
\def\Ugram   {\ensuremath{\rm \,g}\xspace} %kg
% for energy
\def\eV   {\ensuremath{\rm \,eV}\xspace} %eV
\def\UJoule   {\ensuremath{\rm \,J}\xspace} %Joule
% for time
\def\Uminute {\ensuremath{\rm \,min}\xspace} %minute
\def\Uhour {\ensuremath{\rm \,hour}\xspace} %year
\def\Uyear {\ensuremath{\rm \,yr}\xspace} %year
% for frequency
\def\Hz   {\ensuremath{\rm \,Hz}\xspace} %Hz
% for charge
\def\UCoulomb   {\ensuremath{\rm \,C}\xspace} %Coulomb
\def\UmuC   {\ensuremath{\rm \,\upmu{}C}\xspace} %muC
\def\UmegaC   {\ensuremath{\rm \,MC}\xspace} %muC
% for current
\def\UAmpere {\ensuremath{\rm \,A}\xspace} %Ampere
% for electrical potential
\def\UVoltage   {\ensuremath{\rm \,V}\xspace} %Voltage
\def\UkV   {\ensuremath{\rm \,kV}\xspace} %kV
% for capacity
\def\UFarady   {\ensuremath{\rm \,F}\xspace} %Faraday
\def\UpF   {\ensuremath{\rm \,pF}\xspace} %pF
% for electricity field
\def\UVperm   {\ensuremath{\rm \,V/m}\xspace} %V/m
\def\UkVperm   {\ensuremath{\rm \,kV/m}\xspace} %kV/m
\def\UkVpercm   {\ensuremath{\rm \,kV/cm}\xspace} %kV/cm
\def\UNperC   {\ensuremath{\rm \,N/C}\xspace} %N/C
% for pressure
\def\Uatm   {\ensuremath{\rm \,atm}\xspace} %Atmosphere
% for charge density
\def\UCpermtwo   {\ensuremath{\rm \,C/m^2}\xspace} %C/m^2
% for density
\def\Ugpermthree   {\ensuremath{\rm \,g/m^3}\xspace} %g/m^3
% for electric dipole
\def\UCm{\ensuremath{\rm \,C\cdot{}m}\xspace} %C.m
% for accelerator
\def\Umpersec{\ensuremath{\rm\,m/s^2}\xspace} %m/s^2
% for mol
\def\Umol{\ensuremath{\rm\,mol}\xspace} %mol
\def\Ugmol{\ensuremath{\rm\,g/mol}\xspace} %g/mol

\def\Udps{\ensuremath{\rm\,dps}\xspace} % dps
\def\UmicroCi{\ensuremath{\rm\,microCi}\xspace} % dps

% used to align tables and equations
\newcommand{\xx}{\ensuremath{\kern 0.5em }}
\def\y {\ensuremath{y}\xspace}

% some definition for pPb collisions
\def\pPb {\ensuremath{p\mathrm{Pb}}\xspace}
\def\pA {\ensuremath{p\mathrm{A}}\xspace}
\def\PbPb {\ensuremath{\mathrm{PbPb}}\xspace}
\def\sPlot{\mbox{\em sPlot}\xspace}
\def\sWeight{\mbox{\em sWeight}\xspace}

%\def\lone   {L0\xspace}
%\def\hlt    {HLT\xspace}
%\def\hltone {HLT1\xspace}
%\def\hlttwo {HLT2\xspace}
\def\TOS {TOS\xspace}
\def\TIS {TIS\xspace}


\usepackage{multirow} % for complicated table
\usepackage{booktabs} % for complicated table
\usepackage{rotating}
%%%\usepackage{nuc}


